Clio: A Hardware-Software Co-Designed Disaggregated Memory System

Memory disaggregation has attracted great attention recently because of its benefits in efficient memory utilization and ease of management. So far, memory disaggregation research has all taken one of two approaches: building/emulating memory nodes using regular servers or building them using raw memory devices with no processing power. The former incurs higher monetary cost and faces tail latency and scalability limitations, while the latter introduces performance, security, and management problems. Server-based memory nodes and memory nodes with no processing power are two extreme approaches. We seek a sweet spot in the middle by proposing a hardware-based memory disaggregation solution that has the right amount of processing power at memory nodes. Furthermore, we take a clean-slate approach by starting from the requirements of memory disaggregation and designing a memory-disaggregation-native system. We built Clio, a disaggregated memory system that virtualizes, protects, and manages disaggregated memory at hardware-based memory nodes. The Clio hardware includes a new virtual memory system, a customized network system, and a framework for computation offloading. In building Clio, we not only co-design OS functionalities, hardware architecture, and the network system, but also co-design compute nodes and memory nodes. Our FPGA prototype of Clio demonstrates that each memory node can achieve 100 Gbps throughput and an end-to-end latency of 2.5 us at median and 3.2us at the 99th percentile. Clio also scales much better and has orders of magnitude lower tail latency than RDMA. It has 1.1x to 3.4x energy saving compared to CPU-based and SmartNIC-based disaggregated memory systems and is 2.7x faster than software-based SmartNIC solutions.

==> Makefile <==
MY_DATE := $(strip $(shell date +"%F_%H_%M_%S"))
LATEXDIFF=./latexdiff-so

ifeq ($(OS),Windows_NT)
$(warning Windows NT detected "$(USER)")
DVI = yap
DVIBIN = yap
DISTILL = "$(HOME)"/bin/acrodist.exe

PREFIX=c:\\cygwin\\home\\$(USER)\\papers\\2008SASP-arsenal\\
ACROREAD = "$(HOME)"/bin/acroread.exe
ALL = show_nt
else # mac

ifeq ($(USER),mbt)
ALL = show_nt
ACROREAD = kpdf
else
ALL =  pdf
endif

endif


TEX=$(wildcard *.tex)
TEX_DIFF := $(filter-out paper.tex,$(VAR)) paper_diff.tex
FIGS=$(wildcard Figures/*.pdf)
GRAPHS=$(wildcard Graphs/*.pdf)

PDF_TARGETS= paper.pdf extended-abstract.pdf
GENERATED = draft.tex rev.tex draft.pdf paper.pdf extended-abstract.pdf appendix.pdf diff-preamble.tex diff-preamble-new.tex

.PHONY: test_build clean 

all: $(ALL)

paper_diff.pdf: $(TEX_DIFF) $(GRAPHS) $(FIGS) Makefile paper.bib
paper.pdf:  $(TEX) $(GRAPHS) $(FIGS) Makefile paper.bib
extended-abstract.pdf:  $(TEX) $(GRAPHS) $(FIGS) Makefile paper.bib

paper.ps: paper.pdf
	pdftops paper.pdf paper.ps

singlefile.tex: $(filter-out singlefile.tex,$(TEX))
	echo "" > singlefile.tex
	while read line; do if [ "`echo $$line | grep '^\\input{' | tr '{' ' ' | tr '}' ' ' | awk '{print $$2}'`" == "" ]; then echo $$line >> singlefile.tex; else cat `echo $$line | grep '^\\input{' | tr '{' ' ' | tr '}' ' ' | awk '{print $$2}'`.tex >> singlefile.tex; fi; done < paper.tex

draft.tex: paper.tex Makefile
	perl -ne 's/title\{/title\{r\\input\{rev\}: /g; s/^(\\(numberofauthors|conference|Copy))/\%$$1/; s/texheader/draftheader/g; print' < $< >  $@ || rm -f $@

.PHONY: update_rev
update_rev:
	@REV=$$(svn info * */* 2>&1 | grep "Last Changed Rev" | sort -k4 -n | tail -n 1 | awk '{print $$4}');\
	OLDREV=$$(cat rev.tex);\
	if [ "$$REV" != "$$OLDREV" ]; then svn info * */* 2>&1 | grep "Last Changed Rev" | sort -k4 -n | tail -n 1 | awk '{print $$4}' > rev.tex; fi

.PHONY: draft
draft:
	svn update
	make draft.pdf

draft.pdf: draft.tex update_rev $(TEX) $(GRAPHS) $(FIGS) Makefile paper.bib draftheader.tex


.PHONY: diff git-diff

git-diff:
	test -n "$(REV)"
	latexdiff-vc --flatten --git -r $(REV) paper.tex --pdf

diff: diff-preamble.tex singlefile.tex
	-@rm -rf diffsrc
	-@mkdir -p diffsrc
	@if [ "$$REV" == "" ]; then \
	   echo using head revision, override with REV=1234; \
	   REV=$$(svn info * */* 2>&1 | grep "Last Changed Rev" | sort -k4 -n | tail -n 1 | awk '{print $$4}'); \
	 fi; \
	 SVNURL=$$(svn info | grep URL | awk '{print $$2}'); cd diffsrc; svn co -N -r $$REV $$SVNURL .;
	$(LATEXDIFF) --append-context2cmd="tabcolsep" --flatten --type=UNDERLINE diffsrc/paper.tex paper.tex > diff.tex;
	@mv diff.tex diff2.tex		
	@cat singlefile.tex | grep 'begin{document}' -B99999 | grep -v 'begin{document}' > diff.tex
	@cat diff-preamble.tex >> diff.tex
	@cat diff2.tex | grep 'begin{document}' -A99999 >> diff.tex
	@make diff.pdf
	@rm -rf diffsrc
	@rm diff.tex diff2.tex diff.blg diff.log

diff-new: diff-preamble-new.tex singlefile.tex
	-@rm -rf diffsrc
	-@mkdir -p diffsrc
	@if [ "$$REV" == "" ]; then \
	   echo using head revision, override with REV=1234; \
	   REV=$$(svn info * */* 2>&1 | grep "Last Changed Rev" | sort -k4 -n | tail -n 1 | awk '{print $$4}'); \
	 fi; \
	 SVNURL=$$(svn info | grep URL | awk '{print $$2}'); cd diffsrc; svn co -N -r $$REV $$SVNURL .;
	$(LATEXDIFF) --append-context2cmd="tabcolsep" --flatten --type=UNDERLINE diffsrc/paper.tex paper.tex > diff.tex;
	@cat diff.tex | awk -v RS='(\\\\DIFdelbegin |\\\\DIFdelend )' -v ORS= 'NR%2' > diff2.tex
	@cat singlefile.tex | grep 'begin{document}' -B99999 | grep -v 'begin{document}' > diff.tex
	@cat diff-preamble-new.tex >> diff.tex
	@cat diff2.tex | grep 'begin{document}' -A99999 >> diff.tex
	@make diff.pdf
	@rm -rf diffsrc
	@rm diff.tex diff2.tex diff.blg diff.log

diff.pdf: diff.tex $(FIGURES) $(GRAPHS) Makefile paper.bib


test_build:
	rm -rf _test_build
	mkdir _test_build
	(REPO=$$(svn info | grep URL | sed 's/URL: //');\
	 DIR=$$(svn info | grep URL | sed 's/.*\///');\
	 cd _test_build; \
	 svn checkout $$REPO;\
	 cd $$DIR;\
	 make;\
	 open paper.pdf;\
	)	

%_abbrv.bib: %.bib
	./abbrv.py $< $@

pdf: $(PDF_TARGETS)

%.aux : %.tex $(TEX_STUFF)
	pdflatex $(PDFLATEX_BATCH_OPTIONS) $* 

%.bbl : %.aux 
	bibtex $* || true

%.pdf : %.bbl
	pdflatex $(PDFLATEX_BATCH_OPTIONS) $*
	pdflatex $(PDFLATEX_BATCH_OPTIONS) $*

#
# copies file to prevent write-after-read problems
# uses date as suffix.
#
show_nt: pdf
	- killall $(ACROREAD)
	cp paper.pdf paper_$(MY_DATE).pdf
	$(ACROREAD) $(PREFIX)paper_$(MY_DATE).pdf &

clean:
	rm -rf *.aux *.log *.bbl *.blg *.out $(GENERATED)
	rm -rf paper_abbrv.bib 
	rm -rf _test_build

.PHONY: mailme
mailme: draft.pdf pdf
	@REV=$$(svn info * */* 2>&1 | grep "Last Changed Rev" | sort -k4 -n | tail -n 1 | awk '{print $$4}');\
	CLEAN=$$(if [ "`svn diff | wc -l`" == "0" ]; then echo ""; else echo " modified"; fi);\
	EMAIL=$$(finger `whoami` | head -n1 | tr ' ' '\n' | grep @ | tr '<' ' ' | tr '>' ' ');\
	URL=$$(svn info | grep URL | head -n1);\
	URLSHORT=$$(echo $$URL | tr '/' '\n' | tail -n 1);\
	echo -e "Paper from\n$$URL\nRev: $$REV $$CLEAN\nBuild: $$(date)" | mutt -s "Paper $$URLSHORT @ $$REV $$CLEAN" -a paper.pdf -a draft.pdf $$EMAIL;\
	echo Paper emailed to $$EMAIL



diff-preamble.tex: Makefile
	@echo '\RequirePackage[normalem]{ulem}                                 ' > $@
	@echo '\providecommand{\DIFadd}[1]{{\protect\color{blue}\uwave{#1}}}   ' >> $@
	@echo '\providecommand{\DIFdel}[1]{{\protect\color{red}\sout{#1}}}     ' >> $@
	@echo '\providecommand{\DIFaddbegin}{}                                 ' >> $@
	@echo '\providecommand{\DIFaddend}{}                                   ' >> $@
	@echo '\providecommand{\DIFdelbegin}{}                                 ' >> $@
	@echo '\providecommand{\DIFdelend}{}                                   ' >> $@
	@echo '\providecommand{\DIFaddFL}[1]{\DIFadd{#1}}                      ' >> $@
	@echo '\providecommand{\DIFdelFL}[1]{\DIFdel{#1}}                      ' >> $@
	@echo '\providecommand{\DIFaddbeginFL}{}                               ' >> $@
	@echo '\providecommand{\DIFaddendFL}{}                                 ' >> $@
	@echo '\providecommand{\DIFdelbeginFL}{}                               ' >> $@
	@echo '\providecommand{\DIFdelendFL}{}                                 ' >> $@


diff-preamble-new.tex: Makefile
	@echo '\RequirePackage[normalem]{ulem}                                 ' > $@
	@echo '\usepackage{comment}                                            ' >> $@
	@echo '\excludecomment{DIFdelregion}                                   ' >> $@
	@echo '\providecommand{\DIFadd}[1]{{\protect\color{blue}\uwave{#1}}}   ' >> $@
	@echo '\providecommand{\DIFdel}[1]{{\protect\color{red}\sout{#1}}}     ' >> $@
	@echo '\providecommand{\DIFaddbegin}{}                                 ' >> $@
	@echo '\providecommand{\DIFaddend}{}                                   ' >> $@
	@echo '\providecommand{\DIFaddFL}[1]{\DIFadd{#1}}                      ' >> $@
	@echo '\providecommand{\DIFdelFL}[1]{\DIFdel{#1}}                      ' >> $@
	@echo '\providecommand{\DIFaddbeginFL}{}                               ' >> $@
	@echo '\providecommand{\DIFaddendFL}{}                                 ' >> $@
	@echo '\providecommand{\DIFdelbeginFL}{}                               ' >> $@
	@echo '\providecommand{\DIFdelendFL}{}                                 ' >> $@

.PHONY=rubber
rubber: *.tex *.bib
	rubber --pdf paper.tex




==> asplos-intro.tex <==
\section{Introduction}
\label{sec:introduction}

Modern datacenter applications like graph computing, data analytics, and deep learning have increasing demand for access to large amounts of memory.
Unfortunately, server machines are facing {\em memory capacity walls} because of pin, space, and power limitations~\cite{HP-MemoryEvol,ITRS14,MemoryWall95}.
Going forward, it is imperative for datacenters to seek solutions that can go beyond what a (local) machine can offer, \ie, using non-local memory.

At the same time, datacenters are seeing the needs from management and resource utilization perspectives
to {\em disaggregate} resources --- separating hardware resources into different network-attached pools 
that can be scaled and managed independently.
Disaggregated memory pool is thus an appealing proposal that has recently been 
seriously considered by several datacenter providers.
However, although many major datacenters have successfully adopted disaggregated storage systems~\cite{FACEBOOK-BRYCECANYON,FB1,AMAZON-S3,AMAZON-EBS,SnowFlake-NSDI20,Ali-SinglesDay},
it is unclear how to best build {\em disaggregated memory systems},
as memory and storage systems have fundamentally different interfaces and performance requirements.

Disaggregated memory proposals so far have taken two main approaches.
The first type treats the disaggregated memory pool as a {\em passive} party 
(raw, physical memory space with no processing power),
and the compute pool manages the memory pool and provides high-level services to 
applications~\cite{HP-TheMachine,Tsai20-ATC,Lim09-disaggregate,Nitu18-EUROSYS,Genz-citation}.
The main problem of passive disaggregation is the addition of excessive network RTTs
when completely separating processing and memory.

The second type runs management and service software at the memory pool~\cite{InfiniSwap,NAMDB,Kalia14-RDMAKV,Aguilera18-ATC}
to avoid the high-RTT problem of passive disaggregated memory. 
%Co-locating management with memory reduces network RTTs.
%organizes the disaggregated memory pool with regular servers and runs all or part of management software 
%at these servers' CPUs
This type can be considered as {\em software-based active} disaggregated memory ({\em \sadm}), 
and the software can run either at a CPU of a regular server %(server-based)
or at low-power cores in a device like an ARM-based SmartNIC.
For the former, using whole servers to build the memory pool significantly increases owning and energy cost compared to non-disaggregated systems.
%, with full servers and large amounts of CPU cycles at the memory layer.
Moreover, the number of CPU cores limits the amount of parallel memory requests a memory server can handle.
For the latter, %An alternative way of building active disaggregated memory is to run management software in low-power cores.
low-power cores cannot meet the high-bandwidth and low-latency demands of memory systems~\cite{Tsai20-ATC}.

In short, existing disaggregated memory proposals have either performance or cost problems.
\if 0
Another fundamental issue of these existing systems is their reliance on RDMA (Remote Direct Memory Access).
%Albeit its superior performance, RDMA's limited interface is too restrictive for most applications,
%giving rise to several recent proposals of hardware~\cite{StRoM,Aguilera-FarMemory} and software~\cite{Tsai17-SOSP,HyperLoop} extensions to RDMA.
RDMA and RDMA-based systems are an ill fit for memory disaggregation because the RDMA protocol and implementation are both tightly bound with the processor that co-locates with the memory.
At least a process running on this processor needs to perform virtual memory allocation 
and registration through an OS and then share the allocated virtual memory addresses
with other (client) servers that wish to access the allocated memory. 
Essentially, RDMA's abstraction is a {\em host-server-centric} memory view.
%RDMA's interface is virtual memory addresses allocated by processes running at the server where the data is; 
%these addresses need to be shared to other servers for clients to use.
%This addressing mode forces RDMA memory to attach to a host CPU and host software.
What fits disaggregated memory is a {\em client-centric} memory view 
where client applications running on a server can directly access remote memory without the need to contact or maintain 
any additional processes or OSs running at the memory side.
%that enables remote memory to be independent of a host-server.
%With \phdm, remote memory is directly addressed by client-side application processes' virtual address spaces.
%Moreover, a client-side address space in \phdm\ could span multiple \MN{}s. %memory nodes.
\fi
We propose a {\em hardware-based active disaggregated memory} ({\em \phdm}) model.
Like \sadm, %software-based active disaggregated memory, 
\phdm\ performs management and service tasks at the memory pool.
Unlike \sadm, \phdm\ uses customized hardware at the disaggregated memory to achieve performance goals and to avoid the high owning cost of full servers.
%\zhiyuan{
%Unlike \sadm, \phdm\ uses specialized hardware to attach disaggreated memory banks direcly to datacenter network, avoids the high owning cost and interconnect overhead for full servers.
%}
Further, unlike RDMA-based solutions, applications running on {\em compute (client) 
nodes} ({\em \CN}s) can store data in any set of disaggregated {\em memory nodes}
({\em \MN}s) and access them via a sinale client-centric memory space.
Finally, we propose to use programmable hardware 
to enable flexible implementation and deployment of different distributed memory services.
%virtualize and orchestrate disaggregated memory accesses,
%3) provides high-level distributed memory services, 
%and 4) supports changing/adding/removing services through programmable hardware.
%Applications running on {\em compute (client) nodes} ({\em \CN}s) store and access data 
%in a set of disaggregated {\em memory nodes} ({\em \MN}s).
%\MN{}s are programmable hardware devices directly connected to the network,
%each managing its own memory and collectively providing one or more remote distributed memory services.

The \phdm\ model offers several benefits that are key to meeting today's datacenter needs.
With a separate, self-contained remote memory layer, 
\phdm\ makes it easy to configure, manage, and scale remote memory.
With a (good) hardware-based implementation, remote memory services can achieve
high-bandwidth, low-latency performance 
and support large amounts of clients in parallel.
By offering high-level distributed memory services, 
applications can easily use remote memory without 
worrying about its distributed nature or dealing with low-level interfaces.
Finally, programmable hardware enables the reuse of the same hardware for different 
types of memory services, yielding faster and cheaper deployment. %option than ASIC.

We built {\em \sys},
an \phdm\ system %and the first publicly described hardware implementation of disaggregated memory.
%that %offers many benefits over existing remote-memory solutions.
that delivers {\bf hardware-like performance and software-like flexibility, within a tight cost budget}.
\sys's high-level ideas are to extend traditional virtual memory systems to a distributed one 
and to separate data and metadata virtual memory operations by running the former in hardware and the latter in low-power processors.
%traditional execute the data plane in hardware
%and the metadata and control planes in low-power ARM cores.
Each \sys\ cluster consists of 1) a set of \CN{}s that run user applications on top of a \sys\ user-level library,
2) a set of \MN{}s, each being a network-attached hardware device with FPGA, 
an ARM processor, and large amounts of DRAM,
and 3) one {\em global controller}, a regular server that oversees the whole
cluster (Figure~\ref{fig-arch}).
%performs monitoring, orchestration, 
%and coarse-grain metadata operations for the whole cluster.
%Figure~\ref{fig-arch} demonstrates this overall architecture.
Each application process running on a \CN{} has its own {\em remote} virtual memory address space.
%that is separated from its regular local address space.
Physical memory in this address space can sit on multiple \MN{}s,
and the physical locations are hidden from applications.
Similar to traditional address spaces, \sys\ protects remote address spaces from each other.
%but a remote virtual memory address space can map to physical memory on multiple \MN{}s.

There are three key technical challenges \sys\ faces.
First, {\em how to ensure low-latency, high-throughput end-to-end performance} 
when not every operation is implemented in hardware (because of flexibility and cost budget)?
Our key idea is to implement data operations in hardware pipelines with guaranteed 
{\em performance determinism} and to move metadata operations and 
non-performance-deterministic operations off performance-critical path 
to run in software (at each \MN's ARM processor and the global controller).
%We implement \sys's data plane an FPGA and metadata plane in software that runs at the global controller and each \MN{}'s ARM processor.
Further, we use a novel, asynchronous approach to efficiently interact between 
the data plane and the (slower) metadata plane.
With these ideas, we implemented a new page table design, a new page-fault handler,
a reliable network stack, and other virtual memory operations 
in FPGA hardware and software.
%a virtual-to-physical memory address translation unit,
%and a page fault handler, and logic to access memory data.
%We implement the metadata plane in software that runs at the global controller and each \MN{}'s ARM processor.
%They perform virtual and physical memory allocation, monitoring, and load balancing.

Second, {\em how to make a virtual memory system distributed?}
%At the core of \sys\ is a remote distributed virtual memory system.
\sys's answer is a two-level approach, % to manage distributed memory, 
where the global controller assigns {\em coarse-grain} remote virtual memory address ranges to \MN{}s
and each \MN\ manages its virtual and physical memory at fine granularity.
Further, instead of traditional swap-based paging, we %propose %migration-based approaches
use a novel approach that leverages the distributed nature of \sys\ memory to {\em migrate} memory across \MN{}s
during space or load pressures.
%for on-demand memory allocation% and load balancing. %, and memory redundancy.

Finally, {\em how to support flexible extension of distributed services?}
On top of \sys's main functionalities, 
we built a framework for implementing and running extended memory services.
Each extended service's data plane is encapsulated in a {\em module} on the FPGA,
with its own protection domain and virtual address space.
% (that is orthogonal to user application processes).
These modules can directly use \sys's virtual memory data/metadata APIs and distributed operations, %, distributed operations, and 
or implement their own counterparts but leverage \sys's general framework. %(\eg, by building 
Thus, developing extended memory services on \sys\ is easier than on raw hardware but still flexible.

We implemented \sys\ on a low-cost Xilinx FPGA+ARM board,
and we built %several extended virtual memory APIs including pointer operations, \fixme{XXX}, and \fixme{XXX},
two distributed memory services: a shared multi-version data store, {\em \sysmv},
and a distributed in-memory key-value store, {\em \syskv}.
\sys\ achieves network line-rate throughput 
and an end-to-end read/write latency of 2.4--2.6\mus.
%We compare \sys\ and \syskv\ with a passive disaggregated memory system,
%a \sadm\ system, % (running on CPU and on ,
%and raw RDMA.
It outperforms the best existing passive diaggregated memory system by 23\%
and a popular CPU-based \sadm\ system by 29\%.
%Compared to server-based disaggregated memory systems, 
\sys\ also has a 2\x\ owning cost and 25\x\ energy cost savings over server-based disaggregated memory systems.
Overall, this paper makes the following contributions.

\begin{itemize}

\item The first publicly described disaggregated memory system built with real (non-server) hardware.

\item A design that separates memory systems' data and metadata planes into hardware and software.

\item A distributed virtual memory system that integrates hardware and software in novel ways.

%\item Hardware-based distributed operation support such as migration and replication.

\item A framework to build extended memory services %on virtual memory interface
and two hardware-based distributed memory services.
% and a set of extended virtual memory APIs. 
%\item Demonstration of how real systems could use and benefit from disaggregated memory services.

%\item Two hardware-based high-level distributed memory services.
%\item Demonstration of two deployment models of disaggregated memory hardware.

\end{itemize}



==> extended_abstract.tex <==


%\documentclass[pageno]{jpaper}

%replace XXX with the submission number you are given from the ASPLOS submission site.
%\newcommand{\asplossubmissionnumber}{968}

%\usepackage[normalem]{ulem}
%\input{macros}
%\input{defs}
%\usepackage[numbers,sort]{natbib}

%\begin{document}

\title{Clio: A Hardware-Software Co-Designed Disaggregated Memory System \\ \textbf{Extended Abstract}\vspace{-0.3in}}

\date{}

\maketitle

\thispagestyle{empty}

%\section{Introduction and Motivation}
%\label{sec:intro}






\section{Motivation}

Modern data-center applications like graph computing, data analytics, and deep learning have increasing demand for access to large amounts of memory~\cite{FastSwap}.
Unfortunately, servers are facing {\em memory capacity walls} because of pin, space, and power limitations~\cite{HP-MemoryEvol,ITRS14,MemoryWall95}.
Going forward, it is imperative for datacenters to seek solutions that can go beyond what a (local) machine can offer, \ie, using remote memory.
At the same time, data centers are seeing the needs from management and resource utilization perspectives
to {\em disaggregate} resources~\cite{Ali-SinglesDay,SnowFlake-NSDI20,FB1}\textemdash separating hardware resources into different network-attached pools 
that can be scaled and managed independently.
These real needs have pushed the idea of memory disaggregation ({\em \md} for short):
organizing computation and memory resources as two separate network-attached
pools, one with compute nodes ({\em CN}s) and one with memory nodes ({\em MN}s).

\section{Limitations of the State of the Art}
So far, \md\ research has all taken one of two approaches,
building/emulating \MN{}s with either regular servers~\cite{AIFM,InfiniSwap,FastSwap,Shan18-OSDI,zombieland} 
or raw memory devices with no processing power~\cite{Tsai20-ATC,Lim09-disaggregate,Lim12-HPCA,HP-TheMachine}.
%,ATC21Paper
%\textit{Is it possible to build \MN{}s without a server}, as promised by the original proposal of \md~\cite{Lim09-disaggregate,Shan18-OSDI}?
The fundamental issues of server-based approaches such as RDMA-based systems are the monetary cost of a host server and the inherent performance and scalability limitations caused by the way NICs interact with the host server's virtual memory system.
Raw-device-based solutions have low costs.
However, they introduce performance, security, and management problems
because when \MN{}s have no processing power, all the data and control planes have to be handled at \CN{}s~\cite{Tsai20-ATC}.
%\MN{}s become too ``dumb'' and low level when removing its processing power altogether.
%overhead of root cause why RDMA is unfit for \md\ is that it is designed to work around a host server,
%and traditional servers' virtual memory system is not designed for \md.
%Contrary to server-based \md\ solutions, \pdm\ is another extreme where there is no processing at all at \MN{}s.
%The root cause of \pdm's various performance, security, and management problems is exactly this: 
%\MN{}s are too ``dumb'' and low level.

%From the above discussion, we find that both server-based \md\ and raw physical \md\ have their limitations.
Server-based \MN{}s and \MN{}s with no processing power are two extreme approaches of building \MN{}s.
We seek a sweet spot in the middle by proposing a hardware-based \md\ solution that has the right amount of processing power at \MN{}s.
%for the right type of \MN{} management system.
%To mitigate RDMA's various issues for \md, one could try to improve RDMA's hardware design or add a software layer to work around RDMA's problems.
%This paper takes a different approach by starting
Furthermore, we take a clean-slate approach by starting from the requirements of \md\
and designing a \md-native system.
%LegoOS is the only existing work that also proposes a .
%Unfortunately, LegoOS still uses server software and the RDMA network to emulate its hardware design, leaving all the research questions we ask in this paper unanswered.

\section{Key Insights and Proposal}

\input{fig-architecture}

We built {\em \sys}, a hardware-based disaggregated memory system (Figure~\ref{fig-arch}).
%focusing on the hardware-based virtual memory system and network stack.
\sys\ includes a \CN-side user-space library called {\em \syslib}
and a new hardware-based \MN\ device called {\em \sysboard}.
Multiple application processes running on different \CN{}s could allocate memory from the same \sysboard, with each process having its own {\em remote virtual memory address space}.
Applications access their remote memory space using APIs that \sys\ provides (\eg, \alloc, \sysread, \syswrite, \syslock), and the accesses are in byte granularity.
For each API, \sys\ provides a synchronous version and an asynchronous version, with the former following sequential consistency and the latter following release consistency.

A \sysboard\ consists of three main components: 1) a hardware chip that integrates a thin network stack and a virtual memory system to handle data requests (the {\em fast path}), 2) an ARM processor that runs software to handle metadata requests and background tasks (the {\em slow path}), and 3) an FPGA that hosts application computation offloading (the {\em extend path}).

In building \sys, we explore new requirements, challenges, and benefits of \md.
Specifically, we answer three important research questions.

First, \textbf{how does the design and implementation of a
dedicated hardware \MN\ differ from server and programmable NIC
designs?}
%To protect the accesses from different applications to the memory in an \MN\ and to make such accesses flexible, 
%we should use a virtual memory system to check and map virtual memory addresses to physical addresses.
Current \md\ solutions rely on a host server (its OS and MMU) to provide a virtual memory system so that accesses to the memory are protected and flexible. 
Using a whole server just for the virtual memory system is overkill and unnecessarily adds monetary and energy costs to \md. %consumes too much power.
Another possibility is to use a low-power processor (\eg, ARM) in a SmartNIC to run the virtual memory system~\cite{iPipe}. 
However, doing so has high performance impact mainly because the virtual memory system is on a separate chip from the NIC.
%However, doing so has performance overhead, both because the virtual memory system is on a separate chip from the NIC
%and because the virtual memory system is not designed for \md.
%To date, there has been no attempt
%\yizhou{I think here we should emphasize that: MNs emulated using host server has cost and power waste while the SmartNIC-based ones have perf issue. In all, there is no ideal solution for building real server-less MNs. Hence we took a ...}
Overall, server-based approaches have cost overheads while SmartNIC solutions have performance overheads.
We took a clean-slate approach by building a hardware-based virtual memory system that is integrated with a customized hardware network stack, 
both of which are designed specifically for handling virtual memory requests sent over the network.

Second, \textbf{how can a low-cost \MN\ host TBs of memory and support thousands of concurrent application processes?}
Different from traditional (local) memory, an \MN\ is intended to be shared by many applications running at different \CN{}s,
and the more applications it can support, the more efficiently its memory can be utilized.
Thus, we aim to have each \MN\ host TBs of memory for thousands of concurrent applications processes.
However, a hardware design is constrained by the limited resources in a hardware chip such as on-chip memory.
Compared to traditional software-based virtual memory systems, 
how can an \MN\ use orders of magnitude less resources while achieving orders of magnitude higher scalability?
%which raises the problem of how to manage the scalability we target in hardware.
%is especially accute in an \hdm\ because of its low cost requirements.
Current solutions like RDMA NICs swap metadata between NIC's on-chip memory and host server memory,
which comes with performance overhead (4\x\ compared with when metadata is in the NIC memory~\cite{Pythia}).
%RDMA improves scalability by adding more hardware resources to cache more metadata/states), which comes with increasing monetary and energy costs.

Our clean-slate approach is to carefully examine each virtual-memory and networking task 
and to redesign them to \textbf{1)} eliminate states and metadata whenever possible (\eg, by eliminating the RDMA "Memory-Region" concept),
\textbf{2)} move complex but non-performance-critical states, metadata, and tasks to the software slow path,
\textbf{3)} shift functionalities to the \CN\ (\syslib) to reduce \MN's complexity 
(\eg, our reliable network transport runs at \syslib, and \MN\ is ``transport-less''; we achieve reliability by ordering and retrying at the memory request level instead of the packet level),
and \textbf{4)} design bounded-size, inherently scalable data structures (we propose a new page table design that lets all processes share one global page table whose size is determined by the physical memory size).
%For the remaining functionalities that still need caching, we redesign them to guarantee good cache-miss performance.
As a result, each \MN\ (\sysboard) could support TBs of memory and thousands of application processes with only 1.5\MB\ on-chip memory.
%\yizhou{On top of network scalability, I think its also worth explaining how we are able to support TBs of memory. Because this reminds me of O(1) memory issues. With TBs of memory, the memory related metadata and OPs increased as well. Our pros: our fast path use huge page + hashtable-based pgtable, bounded latency. Our cons: our buddy allocator running in ARM is still prone to this huge memory issue.}
%For certain functionalities, we avoid states and metadata alltogether by re-designing the functionalities.
%For functionalities that could be and move the ones that can be moved to the \CN\ side.
%and not relying on cache for good performance.

Third, \textbf{how to minimize tail latency in a \md\ system}?
%\textbf{is it possible to minimize tail latency by processing all read/write requests deterministically?} 
Tail latency is important in data centers especially for workloads that have large fanouts (\eg, Spark jobs).
Although much effort has focused on improving the network and core scheduling for low tail latency~\cite{nanoPU,Shenango,Shinjuku,ZygOS,RPCValet},
the memory system has largely been overlooked.
However, the (remote) memory system is what contributes to extreme long tails in a \md\ system.
For example, RDMA's round-trip latency is around 1--2\mus\ in the common case,
but its tail could be as long as 16.8\ms. % (when there is a page fault).
%The main reason for RDMA's various tails is its reliance on the host virtual memory system, which is not designed for \md\ or for low tail latency.

We reexamine traditional memory system
%from the tail latency and perspectives 
and propose a set of novel mechanisms to bound \sys's tail latency.
Our core idea is to include {\em all} the functionalities that are needed to fulfill all types of data requests in one hardware pipeline
and to make this hardware pipeline {\em performance deterministic}.
This pipeline takes one incoming data unit every cycle (\ie, no pipeline stalls) and completes every request in a fixed number of cycles.
Two major technical hurdles in achieving this performance are to perform page table lookups and to handle page faults in a bounded, short time period.  
For the former, we propose a new {\em overflow-free} hash-based page table that bounds all page table lookups to {\em at most one DRAM access} (instead of the long page table walk in a traditional CPU architecture).
Our novel idea is to avoid overflows at the virtual memory address allocation time, by retrying the allocation until a non-overflow virtual memory address range is found.
For the latter, we propose a new mechanism to handle page faults in hardware with bounded cycles (instead of the costly process of interrupting and handling page faults in OS).

%These mechanisms include 1) handling page faults in hardware,
%2) d
%RDMA’s way is to pre-reserve memory and to use large on-device cache. But cache can’t always work, and reserving memory results in inefficient memory utilization.
%Our solution is to allocate physical memory on-demand and to make the cache miss path fast by handling page faults in hardware and by designing a new hash-based page table. We also carefully designed our hardware pipeline to have deterministic, bounded latency.

\section{Main Artifacts and Key Results}

\input{fig-board}

We prototyped \sysboard\ with a Xilinx MPSoC FPGA board~\cite{ZCU106} and implemented \syslib\ as a user-space library on Linux servers. 
Figure~\ref{fig-coremem} illustrates the overall board-level design.
We built three applications using \sys:
a FaaS-style image compression utility, a radix-tree index, and a key-value store.
%We prototyped \sys's memory device with FPGA (\sysboard).
%\sys\ achieves high throughput (100\Gbps\ with FPGA prototype), low (tail) latency (XXX\mus\ end-to-end MTU round trip latency), 
%low cost (XXX\x\ energy saving), %and great extendibility,
%and \sys\ scales well with XXX. %eliminates {\em all} scalability bottlenecks in both its memory and network systems.
Our FPGA \sys\ prototype achieves 100\Gbps\ throughput and an end-to-end latency of 2.5\mus\ at median and 3.2\mus\ at 99-percentile.
We compared \sys\ with native RDMA, two RDMA-based disaggregated/remote memory systems~\cite{Tsai20-ATC,Kalia14-RDMAKV}, 
a software emulation of hardware-based disaggregated memory LegoOS~\cite{Shan18-OSDI},
%an FPGA-based RDMA implementation~\cite{StRoM}, 
and a software-based SmartNIC BlueField~\cite{BlueField}.
\sys\ scales much better and has orders of magnitude lower tail latency than RDMA, 
while achieving similar throughput and median latency as RDMA (even with the slower FPGA frequency in our prototype).
\sys\ has 1.1\x\ to 3.4\x\ energy saving compared to CPU-based and SmartNIC-based disaggregated memory systems 
and is 2.7\x\ faster than software-based SmartNIC solutions. 
%We will make \sys\ publicly available upon this paper's publication.


Overall, this paper makes the following contributions.

\begin{itemize}

\item The first publicly described hardware-based disaggregated memory system and an FPGA prototype.

\item A demonstration of how to co-design system software (a full virtual memory system), hardware architecture (memory management unit), and networking stack (a customized reliable network).

\item A demonstration of how to co-design the compute and the memory sides in a disaggregated system.

\item A demonstration of how to separate data and control plane in a virtual memory system for disaggregated memory.

\item Three applications built with real disaggregated memory, with some offloading their computation to memory devices.
%\item Hardware-based distributed operation support such as migration and replication.

% and a set of extended virtual memory APIs. 
%\item Demonstration of how real systems could use and benefit from disaggregated memory services.

%\item Two hardware-based high-level distributed memory services.
%\item Demonstration of two deployment models of disaggregated memory hardware.

\end{itemize}



%\subsection*{Why ASPLOS}
%\label{sec:why-asplos}
\section{Why ASPLOS}
This paper demonstrates how to implement a core OS functionality, the virtual memory system, in hardware in a non-conventional way.
We also demonstrate how to co-design hardware and software.
Thus, this paper fits well with the scope of ASPLOS in
architecture and system.
 
\pagebreak
%\bibliographystyle{plain}
%\bibliography{all-defs,all,personal,all-confs,local,paper}


%\end{document}



==> fig-coremem.tex <==
{
\begin{figure}
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/CoreMem.pdf}}
\vspace{-0.1in}
\mycaption{fig-coremem}{\sys\ Core Memory On-Board Design.}
{
}
\end{center}
\vspace{-0.1in}
\end{figure}
}


==> rdma.tex <==
\section{RDMA Issues and \sys\ Solutions}

{\em Remote Direct Memory Access} (RDMA), a high-speed network technology that allows direct access to memory on a remote server,
has been adopted by several major datacenter\cite{AZURE-RDMA,ALIBABA-RDMA}.
It is also the communication media adopted by most existing remote and disaggregated memory systems~\cite{XXX}. 
However, as this section will present, RDMA --- its interface, memory system, and network protocol --- 
are all ill fits for memory disaggregation (esp. for virtualized disaggregated memory),
and existing workarounds all have their limitations.
\sys\ solves RDMA's issues by redesigning and co-design with the virtualized disaggregated memory model.
Figure~\ref{fig-arch} illustrates the architectural differences between RDMA and \sys.
%RDMA supports both {\em one-sided} and {\em two-sided} communication to remote memory.
%One-sided RDMA allows one machine to directly read and write another machine's memory without involving the latter's CPU.
%Two-sided RDMA works like traditional messaging, involving both sender and receiver CPU.
%with one-sided RDMA being used by systems where remote memory are managed by local (compute) machines~\cite{DPM}
%and two-sided RDMA used by systems where each machine manages its own memory~\cite{Kalia14-RDMAKV,Mitchell13-ATC}.
%With the help of one-sided RDMA and other one-sided network technologies~\cite{GenZ},
%several software systems have been proposed to treat 
%Albeit its superior performance, RDMA's limited interface is too restrictive for most applications,
%Although several recent proposals of hardware~\cite{StRoM,Aguilera-FarMemory} and software~\cite{Tsai17-SOSP,HyperLoop} extensions to RDMA made it more flexible and performant, 

%fine-grained sharing

\subsection{Memory System} 
\label{sec:memory}

\subsubsection{Memory Abstraction}
\label{sec:abstraction}
%\subsubsection{Tight Coupling to Co-Located CPU}

\boldpara{RDMA issue.}
Addressing of memory regions ({\em MR}s) registered with RNIC is through the virtual memory address space of a process running at the memory node
(the registering process, or {\em RP} in Figure~\ref{fig-arch}. 
Before registration, the RP first needs to allocate virtual memory address for the MR,
and after registration, the RP passes its virtual memory address and an \rkey\ assigned by the RNIC to application processes running at client nodes.
Essentially, RDMA's abstraction is not a {\em client-facing} one, creating two main issue.
First, clients need to communicate with the RP to allocate or use MRs, usually through a non-RDMA, out-of-band communication channel,
causing performance overhead.
Second and more severe for memory disaggregation, RDMA's abstraction implies that each memory node needs to have a co-located CPU that runs an RP.

\boldpara{Current solutions and their limitations.}
The current practice of using RDMA to access remote memory is to add a client-side software indirection layer 
to translate client application's view (\eg, process virtual memory addresses, object IDs) to MRs and RP's virtual addresses.
%to translate client application's view (\eg, process virtual memory addresses, object IDs) to MRs and RP's virtual addresses.
This approach involves two mappings: client address to RP virtual address (performed at client node) and RP virtual address to remote physical address (performed at memory node).
Doing so (unnecessarily) adds performance and memory space overhead.

\boldpara{\sys\ solution and benefits.}
\sys\ provides a {\em client-facing} virtual memory view 
where client application processes can directly access disaggregated memory with their virtual memory addresses.
\sys\ only performs one address mapping: application virtual address to remote physical address (done at memory node),
and \sys\ completely gets rid of the need for registering processes or server boxes at memory nodes.
Client applications can directly perform allocation, read, write, atomic APIs (\eg, \tas, \cas, \fence), 
and extended APIs like array indexing and pointer chasing (\S\ref{sec:extendability}) to disaggregated devices.

Note that the application ``virtual memory addresses'' \sys\ use (we call them \textit{\sys\ virtual memory address}es) may not necessarily come from normal process memory address space.
In fact, there are three ways to use \sys, and they have their own interpretation of what \sys\ virtual memory addresses mean,
as illustrated in Figure~\ref{fig-arch}.
First, an application process can explicitly call \sys\ APIs by linking to a \sys\ library which creates a special \textit{\sys\ virtual memory address space}
under the hood. 
The returned addresses of \alloc\ and input addresses of \sysread/\syswrite requests will all be virtual addresses in this space ({\em dvma-vaddr}).
Second, applications can sit on top a remote-memory swap system like FastSwap~\cite{FastSwap} and InfiniSwap~\cite{InfiniSwap},
which uses \sys\ virtual memory addresses as swap partition address ({\em swap-vaddr}) and performs \sys\ read/write to swap in/out disaggregated memory.
Third, a disaggregated compute device like pComponent in LegoOS~\cite{Shan18-OSDI} can integrate \sys\ into its hardware cache controller
and send \sys\ read/write with application processes' virtual addresses ({\em AP-vaddr}) for last-level-cache (called ExCache in LegoOS) misses. 

%Using client process virtual memory addresses also has the benefit that disaggregated memory can potentially be 
%integrated into client machine's memory microarchitecture~\cite{Lim09-disaggregate}.


\stepcounter{principle}
\ulinebfpara{Principle \arabic{principle}:}
\textit{The disaggregated memory abstraction should face client processes}.


\subsubsection{Memory Pinning and Page Faults}
\label{sec:pagefault}

\boldpara{RDMA Issue.}
Because RNICs rely on host machine's MMU and OS for virtual memory system support, they do not have any way to deal with page faults.
As a result, RDMA offers only two options, each having their own problem:
1) allocate and ping physical memory when registering MRs with RNIC, 
or 2) no allocation of physical memory and trap to the OS to handle page faults at first accesses.
Option 1) wastes physical memory space before they are used, 
while option 2) has poor performance for first accesses (and thus long tail latency) 
because of the costly communication between RNIC and the host OS (through interrupts)~\cite{ASPLOS17}.
Figure~\ref{fig-} \fixme{XXX}

\boldpara{Current solutions and their limitations.}
To not waste physical memory or causing high page fault performance overhead, 
one option is \textit{fine-grained pinning} where client application dynamically asks 
the memory process to register/unregister a new MR (and pin/unpin physical memory)  
immediately before and after the remote memory usages.
However, it is difficult to infer or ask programmers to specify first memory accesses, 
and RDMA's costly MR register operations significantly degrades application performance
(in our experiments, sending a network request and registering a new MR take \fixme{XXX} in total).
%Another solution proposed recently~\cite{ASPLOS-17} is to 
Thus, the common practice today~\cite{FastSwap,XXX} is to trade memory space for performancy by 
allocating a big MR and pinging its physical memory before an application starts.
%However, such \textit{coarse-grained pinning}'s resulting memory wastes would be a severe problem in a disaggregated setting, 
%as memory at  and should be used by applications as much as possible.

\boldpara{\sys\ solution and benefits.}
\sys\ completely eliminates pinning (and registering) with a virtual memory system that 
performs on-demand physical allocation and page fault handling --- just like what modern OS's provides,
but without the performance cost of RDMA's page fault mechanism.
The key to achieve this is our efficient implementation of the page fault handler in the memory device's main hardware pipeline.
Our main idea here is to move the slower, more complex, and non-deterministic allocation logic (both virtual and physical memory allocation)
to software running at a co-located low-power core, and to use an asynchronous methods to communicate 
between the software allocator and the hardware page fault handler.
With this novel virtual memory system design, our implementation has a \textbf{constant three-cycle latency of page fault handler}.
Figure~\ref{fig-} \fixme{XXX}
We will present the detailed design of our virtual memory system in \S\ref{sec:}.

\stepcounter{principle}
\ulinebfpara{Principle \arabic{principle}:}
\textit{Efficient space usage and performance can both be achieved by integrating virtual memory system in the hardware pipeline}.


\subsubsection{Memory Region}
\label{sec:mr}

\boldpara{RDMA issue.}
RDMA associates a set of metadata with each MR, namely an ID and two keys (\texttt{lkey} and \texttt{rkey}).
RNIC stores these MR metadata in its SRAM cache, and the memory consumption grows linearly with the number of MRs registered with the RNIC. 
When the SRAM is filled up, RNIC will swap the MR metadata to host memory (thrashing), causing significant performance degradation.
Figure~\ref{fig-} \fixme{XXX}

Another issue with MR is that RDMA uses it as the protection scope.
Thus, each client process needs to have at least one MR,
and if two client processes want to share some memory, the RP has to create a new MR.
In addition, metadata of different MRs share the same RNIC cache,
causing (remote) side channels that can be exploited to infer access patterns of victim clients~\cite{Tsai19-Security}.

\boldpara{Current solutions and their limitations.}
One way to reduce the number of MRs is to register a huge MR before an application starts and use a software layer to 
manange this MR (allocation) and map application memory areas to different parts of the MR.
However, as discussed in \S\ref{sec:pagefault}, huge MR will cause either memory waste or high tail latency (due to page faults),
and a new MR needs to be created for each protection scope.
LITE~\cite{Tsai17-SOSP} uses the OS kernel to register the entire server's physical memory as one MR when the system starts up
and to use a kernel module to allocate physical memory to applications.
LITE suffers from performance overhead of user-level-kernel crossings and all the drawbacks of the \pdm\ model (\S\ref{sec:pdm}).
1RMA~\cite{1RMA} uses a fix-sized region table

\boldpara{\sys\ solution and benefits.}
\sys\ gets rid of MR all together. 
With the per-client-process virtual memory space \sys\ offers, applications can allocate (and share) 
as many memory areas as they want without incuring any performance overhead.
%is all  with arbitrary memory areas in the space (through rmalloc instead of registering MR)
Figure~\ref{fig-} \fixme{XXX}

\stepcounter{principle}
\ulinebfpara{Principle \arabic{principle}:}
\textit{}.

\subsubsection{Page Table}
\label{sec:pte}

\boldpara{RDMA issue.}
RDMA uses page tables created and maintained by host CPU and OS to map MRs (RP virtual addresses) to physical memory.
To speed up page table lookup, RNIC caches hot PTEs (page table entries) in its SRAM.
Similar to the scalability problem of MRs, RDMA performance degrades significantly when cached PTEs fill up the SRAM.
Figure~\ref{fig-} \fixme{XXX}

\boldpara{Current solutions and their limitations.}
The common practice to mitigate RDMA's PTE scalability problem is to use huge pages (\eg, 2\GB),
which effectively reduces the number of PTEs~\cite{FaRM,Tsai17-SOSP,XXX}.
However, with large memory, even huge page PTEs could still fill up RNIC SRAM, 
and when it does, it could take up to four DRAM accesses from the RNIC (over PCIe) to walk a x86 page table and fetch a PTE.

\boldpara{\sys\ solution and benefits.}
We propose a new {\em overflow-free} hash-based page table design that bounds the size of PTEs to physical memory size 
and address translation to at most one DRAM access.
Specifically, we store {\em all} PTEs (from all client processes) in a hash table 
whose size is fixed and proportional to the physical memory size of a disaggregated memory device,
\ie, the hash table has enough entries to cover the entire physical memory (\eg, \fixme{XXX \MB\ for 100\GB\ physical memory and XXX page size}).
The hash value of a virtual memory address and its PID is used as the index to determine which hash bucket in the table the corresponding PTE goes to.
To lookup the page table, we always fetch
% compute its hash value (using the {\em lookup3}~\cite{lookup3-wiki} hash function) 
the entire bucket (with all its slots), in a single DRAM read.

Normally, a hash table with fixed slots will have an overflow problem because of hash conflicts.
We use a novel technique to {\em proactively avoid} hash overflows at virtual address allocation time.
To allocate a new virtual memory page, we keep trying available virtual memory addresses until there is one 
whose hash value would go to a bucket that still has an empty slot.
This allocation process is carried out in software running on an ARM core, while the page table lookup is performed by the hardware pipeline of a \sys\ device.
We trade potential retry overhead at allocation time for better run-time performance and simpler hardware design.
% core-memory implementation.
This overhead is manageable because 1) each retry is fast with our implementation~\cite{sec:metadataplane}, 
2) we employ huge pages, which means fewer pages need to be allocated, 
3) we choose a hash function that has very low collision rate~\cite{lookup3-wiki},
and 4) the \sys\ 64-bit virtual address space is huge.

Figure~\ref{fig-} \fixme{XXX}

\stepcounter{principle}
\ulinebfpara{Principle \arabic{principle}:}
\textit{}.

\subsection{Network System}
\label{sec:network}

\subsubsection{Connection, Reliability, and Ordering}

\boldpara{RDMA issue.}
RDMA's RC (reliable connection) mode, the only mode that supports both RDMA one-sided read and write operations,
is connection-oriented, requiring QPs (send\&receive queue pairs) to be established 
between a sender and a receiver before communication can happen.
RDMA implements its transport layer in hardware (RNIC),
and a reliable transport requires per-connection states.
Like MR and PTE, these states and other QP metadata are stored in RNIC SRAM, 
and QPs, too, have scalability issues.
Figure~\ref{fig-} \fixme{XXX}

\boldpara{Current solutions and their limitations}
A common mitigations to the QP scalability issue is QP sharing, 
where multiple threads in a workload or multiple workloads share a QP~\cite{FaSST}.
However, threads sharing a QP content for locks to use the QP,
and the FIFO order enforced by a QP can cause ``false ordering'' among workloads~\cite{1RMA}.
An alternative method is to use RDMA UD (unreliable datagram) mode.
The main issues with UD are its unreliable communication and 
its only support of two-sided RDMA, which requires the receiving node's CPU to be involved in the communication and thus does not fit the disaggregated memory model.

1RMA~\cite{1RMA} proposed a connection-less approach to perform remote read/write
and to use the reply of read/write requests as the ACK.
It relies on 

\boldpara{\sys\ solution and benefits.}
\if 0
Our insight is that we {\em can} achieve reliability without the need for connection or {\em any} states at the memory devices
by exploiting the {\em asymmetric} nature of memory disaggregation.
Our main idea is to shift all reliability tasks at the client side in software
and only include L1 and L2 in hardware (regular Ethernet NIC at client servers and a standard Ethernet MAC module at memory device hardware).
%and perform {\em all} reliable transport operations at the client side in software (\syslib).

Since all \sys\ operations are in the RPC style initiated by client servers, \ie, sending read/write requests and getting data/response back,
we use the reply as the ACK and matches replies to their corresponding requests using a request ID that is embedded in the packet header.
Each request's packet headers also include sender-receiver addresses, which will be used to construct reply packets. 
With these mechanisms, we essentially have a (unreliable) connectionless transport.
Below, we explain how we add reliability.

Network errors can happen when a packet is corrupted, loss, or reordered.
We use link-/physical-layer error correction like Forward Error Correction and retries that are already available in InfiniBand~\cite{MellanoxOFED} \fixme{and Ethernet???}
to deal with packet corruption, similar to prior practices~\cite{RAIL-NSDI17,FaSST}.
As the link layer does not (\fixme{or rarely?}) drop packets, packet loss is mainly due to buffer overflows in the network.
We control (minimize) packet loss with our client-side, software congestion/flow control mechanism (\S\ref{sec:cc}).
In the rare case of packet loss (either in a \sys\ request or its response), the client-side \syslib\ will fail after a request timeout
and retry the entire \sys\ request.
This leaves us with packet reordering, which is rare in non-multi-path network, but can still happen.

We take three approaches in handling packet reordering.
First, we guarantee that each request/reply is always delivered to upper layers in its entirety 
even when it is split into multiple link-layer packets that can be reordered.
We achieve this simply by using intra-request/reply sequence IDs to mark the proper ordering of packets 
and if needed, reorder them before delivering the request/reply.
Second, we offer synchronous APIs, with which we can guarantee that requests in the same session\footnote{Session is a \sys\ notion of }
is executed one after another. 
Thus, even without ordering guarantees from the network layer, synchronous requests will still be executed in order.
Finally, to offer more aggressive performance optimization, we offer asynchronous APIs, 
where multiple requests can be sent out before their replies are received.
Unlike synchronous requests, network reordering can affect asynchrnous requests' ordering.
We handle asynchronous requests' ordering in \sys\ with two methods:
1) the \syslib\ tracks read-write and write-write dependencies (outstanding read and write requests to the same address)
and issue dependent requests in a synchronous way;
2) we· offer a \fence\ operation, which lets a client process to wait until all outstanding asynchrnous requests have finished.
With these mechanisms, applications can achieve {\em release consistency}.

As a result, \sys\ memory devices completely remove the need for network states and thus all network-related scalability bottlenecks,
and client servers only need regular L2 Ethernet NICs with no NIC scalability issues either.
Figure~\ref{fig-} \fixme{XXX}

\stepcounter{principle}
\ulinebfpara{Principle \arabic{principle}:}
\textit{Efficient end-to-end reliability and stateless memory devices can be and is better achieved by shifting reliability handling to client-side software.}
%with unreliable, connectionless network
%Relaxing strict network reliability and handling reliability at system/application level }.  

\subsubsection{Congestion and Flow Control}
\label{sec:cc}

\boldpara{Issue}
RDMA over Converged Ethernet (RoCE) relies on link-layer Priority Flow Control (PFC~\cite{PFC}) to provide a drop-free substrate.
PFC is a mechanism for switches and NICs to avoid buffer overflow by forcing the immediate upstream entity to pause (through PFC pause frames).
However, PFC has a well-known head-of-line blocking issue and a risk of deadlock that make it infeasible to deploy at large scale~\cite{Zhu15-SIGCOMM}.

\boldpara{Current solutions and their limitations}
A common practice adopted by datacenters is to reduce PFC triggering by adding hardware-based congestion control schemes~\cite{Zhu15-SIGCOMM,hpcc-sigcomm19}
or by switching to a backup TCP network~\cite{RDMA-NSDI21}.
These schemes do not fit our needs, as we 
Recently, 1RMA~\cite{1RMA} proposed to 
two RTT writes

\boldpara{\sys\ solution and benefits.}
RDMA's network protocol treats all endpoints the same, \ie, a symmetric protocol.
We make two insights here.
First, with our design and implementation, a \sys\ memory device' internal throughput is always higher than its port bandwidth.
Thus, there will be no buffer overflow in a \sys\ memory device (\ie, it is faster than the network), 
and there is no memory-side in-cast problem and no need for memory-side flow control.
Second, 
client-side controlled congestion control
reactive, delay-based, window based 
solicitation window for client-side incast

\stepcounter{principle}
\ulinebfpara{Principle \arabic{principle}:}
\textit{}.

\subsection{Extendability}
\label{sec:extendability}

\boldpara{Issue}
limited primitives
bundled network stack and memory system, in a closed system
As a result, datacenters cannot easily deploy new transports~\cite{Homa,NDP,pHost} or congestion-control algorithms~\cite{1RMA,XXX}.

\boldpara{Current solutions and their limitations}

\boldpara{\sys\ solution and benefits.}
\sys\ allows \textit{easy extension} to different network stacks, high-level APIs, and to distributed disaggregated memory
modularized approach, each could be replaced by a new one

\stepcounter{principle}
\ulinebfpara{Principle \arabic{principle}:}
\textit{}.

\subsection{Putting It Together}


==> related.tex <==
\section{Related Work}
\label{sec:related}

disaggregated memory:
LegoOS, DPM, remote region, the Machine

distributed memory:
FaRM, RAMCloud, DSPM

rdma related
extended rdma API

FPGA related:
KV-Direct, Catapult


==> tbl-resource-util.tex <==
{
\begin{table*}[th]\footnotesize
\begin{center}
\begin{tabular}{ p{1.0in} | p{0.3in} |p{0.35in} }

 & \textbf{Logic} & \textbf{Memory} \\
\textbf{System/Module} & \textbf{(LUT)} & \textbf{(BRAM)} \\
\hline
\hline
StRoM-RoCEv2-10G & 39\% & 76\% \\
Tonic-SACK-100G & 48\% & 40\% \\
\hline
\sys\ (Total) & 30\% & 31\% \\
VirtMem & 4.8\% & 3\% \\
NetStack & 2.3\% & 1.7\% \\
\hline
Go-Back-N & 5.8\% & 2.6\% \\

\end{tabular}
\end{center}
\mycaption{tbl-resource-util}{XXX}
{
XXXX
}
%\vspace{-0.1in}
\end{table*}
}

==> tbl-system-cmp.tex <==
{
\begin{table*}[th]
\footnotesize
\begin{center}
%\begin{tabular}{ $p{1.2cm} |{\vrule width 1.6pt} ^p{1.2cm} | ^p{1.2cm} | ^c | ^p{1.2cm} |{\vrule width 1.2pt} ^c | ^c | ^c | ^c}
\begin{tabular}{ p{1cm} || p{1.8cm} 	   | p{1.5cm} 		| p{1.4cm}	  | p{1.2cm} 		| p{2.3cm} | p{1.9cm} 		    | p{0.9cm} | p{1.6cm} 	  }
		Scheme 	  & Abstraction   & VirtMemSys Location &  On-Demand Allocation& Offloading Support 	& Latency & Scalability Bottlenecks & Cost & Management\& Extendibility \\
		%\bf Scheme 	  & \bf Abstraction   & \bf VirtMemSys Location & \bf On-Demand Alloc& \bf Offloading Support 	& \bf Latency & \bf Scalability Bottlenecks & \bf Management Extendability \\
\hline
\ChangeRT{1pt}
		\pdm\   	& Physical	& \CN\ HW/SW	& No		& No		& High Min		& \CN\ coordination & Low & Hard   \\
\hline
		RDMA 		& Memory virtual& \MN\ OS/CPU 	& via host OS& SW		& Low Min, High Tail	& Conn, MR, PTE	& High & Hard   \\
\hline
		LegoOS		& Client virtual& \MN\ SW	& No		& No		& High Min		& \MN\ SW	& Medium & Easy	\\
\hline
%\rowstyle{\bfseries}
		\bf\sys\ 	& \bf Client virtual& \bf \MN\ HW& \bf in HW 	& \bf HW	& \bf Low Min, Low Tail	& \bf None	& \bf Low & \bf Easy    
\end{tabular}
\end{center}
\vspace{-0.15in}
\mycaption{tbl-system-cmp}{Comparison of RDMA, \pdm, and \sys.}
{
SW and HW stands for software and hardware.
}
%\vspace{-0.1in}
\end{table*}
}



==> texfooter.tex <==
  %%%%%%%%%%%%%%%%%%%%%%%%5
%\clearpage
%\pagestyle{empty}
%\input{department}
%\clearpage

%\setstretch{0.8}
%\titlespacing*{\section}{0em}{1ex}{1ex}
%\begin{small}

%\begin{spacing}{0.3}
%\bibliographystyle{abbrv}
\bibliographystyle{plain}
\bibliography{all-defs,all,personal,all-confs,local,paper}

%\end{spacing}
%\end{small}

%\clearpage
%\input{bio}
%\clearpage
%\input{budget}
%\clearpage
%\input{facilities}

\end{document}


==> v1-introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Modern datacenter applications like graph computing, data analytics, and deep learning have increasing demand for access to large amounts of memory.
Unfortunately, server machines are facing {\em memory capacity walls} because of pin, space, and power limitations~\cite{HP-MemoryEvol,ITRS14,MemoryWall95}.
Going forward, it is imperative for datacenters to seek solutions that can go beyond what a (local) machine can offer, \ie, using non-local memory.
At the same time, datacenters are seeing the needs from management and resource utilization perspectives
to {\em disaggregate} resources --- separating hardware resources into different network-attached pools 
that can be scaled and managed independently.
Disaggregated memory pool is thus an appealing proposal that has gain a lot of traction recently. 

Most disaggregated memory systems~\cite{Shan18-OSDI,Tsai20-ATC,InfiniSwap,FastSwap} rely on RDMA (Remote Direct Memory Access) as the communication media.
Even though RDMA enables the direct access of remote memory,
we argue that RDMA and RDMA-based NICs (RNICs) are fundamentallly ill fits for building disaggregated memory.
First, \textit{RNIC's memory accesses} relies heavily on co-located host CPU, host memory controller, and software system running at the host.
%causing performance, scalability, and cost problems.
1) RNIC needs to interact with host CPU in the metadata path {\em and} at times (\eg, during page faults), the data path, resulting in performance overheads.
2) RNIC caches memory metadata (\eg, PTEs, memory region information) in its limited SRAM, making it hard to scale with memory size or memory regions.
Furthermore, the RNIC cache is shared by all client processes, resulting in several types of side channel vulnerabilities~\cite{Pythia}.
3) Because of RDMA, a memory node needs to be equipped with at least a CPU and a memory controller, defeating the cost-saving benefits of disaggregation.
%4) Another subtle related issue is side channel~\cite{Pythia}, which is a result of multiple application processes sharing .
%which is not only unnecessary for disaggregated memory but also incurs performance, scalability, and cost problems.

Second, the \textit{RDMA interface} has a memory view that is contradictory to disaggregated memory.
A client process should be able to access a disaggregated memory pool just like accessing its own virtual memory address space,
and physical memory underneath this virtual space should be able to span multiple memory devices.
Instead, with RDMA, memory at a memory node is addressed using the virtual memory address space of processes running at this memory node;
these addresses are then passed to client processes to be used to access the remote memory.
%to let multiple client processes access.
%when using RDMA to connect client machines to memory nodes, 
%another software indirection layer to map client 

Third, the \textit{RDMA network protocol} is not designed for disaggregated memory environments.
Its protocol is general-purpose and ``symmetric'', treating every end host in the same way.
Its connection-based reliable transport has many well-known scalability~\cite{FaRM,Tsai17-SOSP} and congestion~\cite{Zhu15-SIGCOMM} issues
and would add costs to build disaggregated memory nodes (\eg, for maintaining buffers and complex transport and congestion-control logic).

%Disaggregated memory devices should not need a host CPU or a full-blown server, 
%as it contracdicts the main purpose of disaggregation to save costs.
%At the same time, they need to deliver scalable, low-(tail-)latency performance beyond what today's RDMA architecture can provide.
%When building systems and applications on top of RDMA, 

To solve RDMA's various issues, system designers have proposed many software~\cite{Tsai17-SOSP,HyperLoop,FaRM} 
and hardware~\cite{StRoM} solutions \textit{on top of} RDMA.
However, they are point solutions and do not always work for the disaggregated environment. 
%we should design to avoid the fundamental issues of RDMA.
%RDMA was not designed for disaggregated memory and should not be used as is.
For disaggregated memory pools to have standalone devices that are scalable, performant, and low cost, 
we should build a new solution instead of patching RDMA.
In fact, we are not the first to propose alternatives to RDMA.
Industry consortiums have been developing protocols and specifications of coherent interconnects 
that could be used or extended to connect disaggregated devices~\cite{GenZ,CXL,OpenCAPI,CCIX}.
However, they have their own limitations (\S\ref{sec:}). 
Moreover, none of them have been realized with real systems.

%set up time%
%As a result, before a client server can access memory on a remote server via RDMA, 
%a process running at the remote server needs to {\em register} a {\em memory region} with RNIC,
%which sets up page table entries, protection keys, and locations of the memory region 
%RNIC cannot 
%During runtime,  

We propose \textit{\sys} (\textit{Disaggregated Virtual Memory Access}), a solution that enables client (compute) servers 
to have virtual-memory accesses to standalone disaggregated memory devices.
Client processes access disaggregated memory using their own virtual memory addresses, 
and \sys\ performs address translation and memory management at the memory node, 
all in the standalone memory device without the need for a host machine.
\sys\ includes a memory system and a network system, both of which are redesigned for disaggregated memory.

\sys's memory system encoporates the entire virtual memory system (which used to be implemented in the host OS and host memory controller),
including address translation, virtual and physical memory allocation, and page fault handling.
The main challenge here is to efficiently offload the virtual memory system to the device to achieve ``hardware'' performance without the development and monetary cost
of building complex virtual memory logic in hardware.
Our key idea is to implement {\em all} memory access operations including page fault handling in a {\em deterministic} hardware pipeline 
%with guaranteed 
%{\em performance determinism} and to move metadata operations and 
and metadata and non-deterministic operations in software (running at low-power cores).
We use a novel, asynchronous approach to efficiently interact between 
the hardware data plane and the software metadata plane.
We further propose a new conflict-free hash-based page table design that bounds address mapping to take at most one memory access.
The resulting \sys\ memory system finishes all memory read/write operations within three cycles and at most two memory accesses.
even under page faults and under various scaling dimensions.
%Furthermore, we remove all 

\sys's network system includes a new connectionless transport and purely-client-managed congestion and flow control.
Our key observation here is that client nodes and memory devices should be treated as different parties, 
with the former always being the (active) request initiator and the latter being the (passive) responder.
Thus, we propose an asymmetric network protocol where the memory-side is completely 
{\em stateless} and {\em bufferless} (so as to make memory devices low cost and scalable),
and the compute-side handle states and control congestions.
%Furthermore, user-controlled relaxed ordering 


We prototyped \sys's memory device with FPGA (\sysboard).
\sys\ achieves high throughput (100\Gbps\ with FPGA prototype), low (tail) latency (XXX\mus\ end-to-end MTU round trip latency), 
low cost (XXX\x\ energy saving), and great extendability,
and \sys\ eliminates {\em all} scalability bottlenecks in both its memory and network systems.
We compared \sys\ with RDMA

\if 0
Our design of \sys\ follows the following principles.

The current model of RDMA is to use host hardware (MMU) and software (OS) virtual memory system
and to cache memory information (\eg, PTEs) at the resource-constraint RNIC.
slow both during set up time (\eg, costly memory registration step) and during runtime (\eg, interrupting host CPU to serve page faults).
instead of serving as a cache and relying on host to perform set up tasks, 
the device should be the 
We propose to \textit{offload virtual memory system} to hardware and run it in the same chip as the network stack.
challenge, how to build complex virtual memory operations such as virtual memory space management and allocation
\textbf{Principle 2}: \textit{separating data and metadata in a way that data is not blocked by slower metadata operations}
We data path in hardware and metadata and control paths in software 
arm enough, no need for cpu
\textbf{Principle 3}: \textit{eliminate scalability bottlenecks}
no MR, single page table for all processes
\textbf{Principle 4}: \textit{tail latency }
deterministic pipeline cycles, no buffering
\textbf{Principle 5}: \textit{disaggregated memory's access pattern} that is coarse-grain, compute-node-initiated

%\begin{itemize}[noitemsep,leftmargin=0cm,itemindent=.35cm]
\begin{itemize}

\item A thorough analysis of RDMA's issues and current solutions' limitations under the disaggregated memory environment.

\item A hardware-based virtual memory system that completes a memory request within three cycles and at most two memory accesses even under TLB misses and page faults.

\item A new conflict-free hash-based page table design and a 

\item A network stack 

\item FPGA prototype of \sys\ that can reach 100\Gbps\ throughput and 2.4--2.6\mus\ end-to-end round-trip latency. 

\end{itemize}

\fi

\if 0
Another fundamental issue of these existing systems is their reliance on RDMA (Remote Direct Memory Access).
%Albeit its superior performance, RDMA's limited interface is too restrictive for most applications,
%giving rise to several recent proposals of hardware~\cite{StRoM,Aguilera-FarMemory} and software~\cite{Tsai17-SOSP,HyperLoop} extensions to RDMA.
RDMA and RDMA-based systems are an ill fit for memory disaggregation because the RDMA protocol and implementation are both tightly bound with the processor that co-locates with the memory.
At least a process running on this processor needs to perform virtual memory allocation 
and registration through an OS and then share the allocated virtual memory addresses
with other (client) servers that wish to access the allocated memory. 
Essentially, RDMA's abstraction is a {\em host-server-centric} memory view.
%RDMA's interface is virtual memory addresses allocated by processes running at the server where the data is; 
%these addresses need to be shared to other servers for clients to use.
%This addressing mode forces RDMA memory to attach to a host CPU and host software.
What fits disaggregated memory is a {\em client-centric} memory view 
where client applications running on a server can directly access remote memory without the need to contact or maintain 
any additional processes or OSs running at the memory side.
%that enables remote memory to be independent of a host-server.
%With \phdm, remote memory is directly addressed by client-side application processes' virtual address spaces.
%Moreover, a client-side address space in \phdm\ could span multiple \MN{}s. %memory nodes.
We propose a {\em hardware-based active disaggregated memory} ({\em \phdm}) model.
Like \sadm, %software-based active disaggregated memory, 
\phdm\ performs management and service tasks at the memory pool.
Unlike \sadm, \phdm\ uses customized hardware at the disaggregated memory to achieve performance goals and to avoid the high owning cost of full servers.
%\zhiyuan{
%Unlike \sadm, \phdm\ uses specialized hardware to attach disaggreated memory banks direcly to datacenter network, avoids the high owning cost and interconnect overhead for full servers.
%}
Further, unlike RDMA-based solutions, applications running on {\em compute (client) 
nodes} ({\em \CN}s) can store data in any set of disaggregated {\em memory nodes}
({\em \MN}s) and access them via a sinale client-centric memory space.
Finally, we propose to use programmable hardware 
to enable flexible implementation and deployment of different distributed memory services.
%virtualize and orchestrate disaggregated memory accesses,
%3) provides high-level distributed memory services, 
%and 4) supports changing/adding/removing services through programmable hardware.
%Applications running on {\em compute (client) nodes} ({\em \CN}s) store and access data 
%in a set of disaggregated {\em memory nodes} ({\em \MN}s).
%\MN{}s are programmable hardware devices directly connected to the network,
%each managing its own memory and collectively providing one or more remote distributed memory services.

The \phdm\ model offers several benefits that are key to meeting today's datacenter needs.
With a separate, self-contained remote memory layer, 
\phdm\ makes it easy to configure, manage, and scale remote memory.
With a (good) hardware-based implementation, remote memory services can achieve
high-bandwidth, low-latency performance 
and support large amounts of clients in parallel.
By offering high-level distributed memory services, 
applications can easily use remote memory without 
worrying about its distributed nature or dealing with low-level interfaces.
Finally, programmable hardware enables the reuse of the same hardware for different 
types of memory services, yielding faster and cheaper deployment. %option than ASIC.

We built {\em \sys},
an \phdm\ system %and the first publicly described hardware implementation of disaggregated memory.
%that %offers many benefits over existing remote-memory solutions.
that delivers {\bf hardware-like performance and software-like flexibility, within a tight cost budget}.
\sys's high-level ideas are to extend traditional virtual memory systems to a distributed one 
and to separate data and metadata virtual memory operations by running the former in hardware and the latter in low-power processors.
%traditional execute the data plane in hardware
%and the metadata and control planes in low-power ARM cores.
Each \sys\ cluster consists of 1) a set of \CN{}s that run user applications on top of a \sys\ user-level library,
2) a set of \MN{}s, each being a network-attached hardware device with FPGA, 
an ARM processor, and large amounts of DRAM,
and 3) one {\em global controller}, a regular server that oversees the whole
cluster (Figure~\ref{fig-arch}).
%performs monitoring, orchestration, 
%and coarse-grain metadata operations for the whole cluster.
%Figure~\ref{fig-arch} demonstrates this overall architecture.
Each application process running on a \CN{} has its own {\em remote} virtual memory address space.
%that is separated from its regular local address space.
Physical memory in this address space can sit on multiple \MN{}s,
and the physical locations are hidden from applications.
Similar to traditional address spaces, \sys\ protects remote address spaces from each other.
%but a remote virtual memory address space can map to physical memory on multiple \MN{}s.

There are three key technical challenges \sys\ faces.
First, {\em how to ensure low-latency, high-throughput end-to-end performance} 
when not every operation is implemented in hardware (because of flexibility and cost budget)?
Our key idea is to implement data operations in hardware pipelines with guaranteed 
{\em performance determinism} and to move metadata operations and 
non-performance-deterministic operations off performance-critical path 
to run in software (at each \MN's ARM processor and the global controller).
%We implement \sys's data plane an FPGA and metadata plane in software that runs at the global controller and each \MN{}'s ARM processor.
Further, we use a novel, asynchronous approach to efficiently interact between 
the data plane and the (slower) metadata plane.
With these ideas, we implemented a new page table design, a new page-fault handler,
a reliable network stack, and other virtual memory operations 
in FPGA hardware and software.
%a virtual-to-physical memory address translation unit,
%and a page fault handler, and logic to access memory data.
%We implement the metadata plane in software that runs at the global controller and each \MN{}'s ARM processor.
%They perform virtual and physical memory allocation, monitoring, and load balancing.

We implemented \sys\ on a low-cost Xilinx FPGA+ARM board,
and we built %several extended virtual memory APIs including pointer operations, \fixme{XXX}, and \fixme{XXX},
two distributed memory services: a shared multi-version data store, {\em \sysmv},
and a distributed in-memory key-value store, {\em \syskv}.
\sys\ achieves network line-rate throughput 
and an end-to-end read/write latency of 2.4--2.6\mus.
%We compare \sys\ and \syskv\ with a passive disaggregated memory system,
%a \sadm\ system, % (running on CPU and on ,
%and raw RDMA.
It outperforms the best existing passive diaggregated memory system by 23\%
and a popular CPU-based \sadm\ system by 29\%.
%Compared to server-based disaggregated memory systems, 
\sys\ also has a 2\x\ owning cost and 25\x\ energy cost savings over server-based disaggregated memory systems.
Overall, this paper makes the following contributions.

\begin{itemize}

\item The first publicly described disaggregated memory system built with real (non-server) hardware.

\item A design that separates memory systems' data and metadata planes into hardware and software.

\item A distributed virtual memory system that integrates hardware and software in novel ways.

%\item Hardware-based distributed operation support such as migration and replication.

\item A framework to build extended memory services %on virtual memory interface
and two hardware-based distributed memory services.
% and a set of extended virtual memory APIs. 
%\item Demonstration of how real systems could use and benefit from disaggregated memory services.

%\item Two hardware-based high-level distributed memory services.
%\item Demonstration of two deployment models of disaggregated memory hardware.

\end{itemize}
\fi


==> v1-motivation.tex <==

\input{tbl-system-cmp}

\section{Memory Disaggregation}
\label{sec:motivation}

Resource disaggregation is a notion to separate different types of resources into different pools,
each of which can be independently managed and scaled.
Applications can allocate resources from any available node in a resource pool, resulting in tight resource packing. %regardless of where other types of resources sit.
Because of these benefits, % its manageability, independent scaling, and efficient resource utilization benefits,
many datacenters have adopted the idea of disaggregation, often at the storage 
layer~\cite{FACEBOOK-BRYCECANYON,FB1,SnowFlake-NSDI20,AMAZON-S3,AMAZON-EBS,Ali-SinglesDay}.
%layer~\cite{FACEBOOK-BRYCECANYON,FB1,SnowFlake-NSDI20,Decibel-NSDI17,AMAZON-S3,AMAZON-EBS,Klimovic18-ATC,RackScaleDisaggregation}.
%As a recent success story, Alibaba listed their storage disaggregation as one of the five reasons
%that enable them to serve the peak load of 544,000 orders per second on the 2019 Single's Day~\cite{Ali-SinglesDay}.
With the success of disaggregated storage and the fast developments in datacenter network speed,
researchers in both academia and industry started to seek ways to disaggregate memory 
(and persistent memory)~\cite{Lim09-disaggregate,FireBox-FASTKeynote,IntelRackScale,Lim12-HPCA,Shan18-OSDI,RAMCloud,Tsai20-ATC,AIFM,FarMem,InfiniSwap,Semeru}.
Different from distributed memory such as distributed shared memory~\cite{Shasta,Bennett90-PPOPP,Fleisch89-SOSP,Keleher92-ISCA,Grappa},
the disaggregated memory model has a clear notion of function separation where the memory pool hosts memory
and the compute pool executes applications.

\subsection{Requirements of Memory Disaggregation}
Many applications can benefit from disaggregated memory, and their usages can be categorized into two types:
as dynamically allocated memory space (\eg, as part of a heap~\cite{Semeru}, as a swap space~\cite{InfiniSwap}) during the execution of an application,
and as the cache of a data store~\cite{XXX} or the data store itself~\cite{RAMCloud}.
In general, memory disaggregation has the following requirements.

\stepcounter{reqs}
\boldpara{R\arabic{reqs}: Low cost and easy deployment.}
Although disaggregated memory pool can be built with regular servers 
(in fact, most of today's disaggregated memory solutions~\cite{AIFM,FarMem,InfiniSwap,Semeru} are server-based),
it is much cheaper to build and run standalone disaggregated memory devices without a server box or a CPU.
To ease the adoption of disaggregated memory in current datacenters, ideally, there should be no hardware change or addition at client servers.

\stepcounter{reqs}
\boldpara{R\arabic{reqs}: Low-latency and high-throughput.}
Accesses to disaggregated memory are over the network, which is inevitably slower than accessing local memory.
Despite this nature, memory disaggregation should still offer attractive performance, and by offering more (but slower) memory,
overall application performance could be better than with just local memory.
Specifically, when used as dynamically allocated memory, disaggregated memory should deliver low latency so as not to slow down application execution much.
When it is used as (cache of) data store, throughput is more important, 
and accesses to disaggregated memory should reach network line rate.

\stepcounter{reqs}
\boldpara{R\arabic{reqs}: Low tail latency and predictable performance.}
One of the obstacles to adopting disaggregated memory is the fear for unpreditable performance and much worse tail latency than local memory. %, \eg, during network congestion
In addition to network unstability, we found that memory systems could also contribute to long tails with today's RDMA-based systems (\S\ref{sec:}).
Having predictable, bounded performance and low tail latency would be one key to the successful adoption of memory disaggregation in data centers,
where SLAs are important.

\stepcounter{reqs}
\boldpara{R\arabic{reqs}: Scale with clients and memory.}
To fully exploit the resource-utilization benefit of disaggregation, we should allow many client servers and client processes running on them to access and share a memory device.
At the same time, each memory device could host hundreds GBs to few TBs of memory that is expected to be close to fully utilized (and thus bringing down the number of 
memory devices and total cost of a cluster).
Furthermore, we should have no restriction on how applications use the memory, which could result in many disjoint memory regions.
Thus, disaggregated memory should scale with client servers, client processes, memory size, and memory regions.
%each client process should be able to access large amounts of memory and many disjoint memory regions 
%scale with client servers, client processes, memory size, memory regions

\stepcounter{reqs}
\boldpara{R\arabic{reqs}: Independent resource pool management.}
A major reason behind the successful adoption of disaggregated storage at production scale and the traction of disaggregation in general
is its ease of management, as it is more flexible to manage disaggregated resource pools independently at where the resource is.
Memory disaggregation should also follow the practice by managing the disaggregated memory pool.
Datacenter operators can then configure disaggregated memory pool (\eg, adding replication, migrating data across memory nodes)
without affecting other pools.

\stepcounter{reqs}
\boldpara{R\arabic{reqs}: Secure access.}
When deployed in datacenters, it is important to protect disaggregated memory from undesired or malicious accesses.
Disaggregate memory can be shared by many client servers and applications over the network.
It should provide at least the same level of safety guarantees as today's normal (local) memory
and potentially also guard against new security threasts such as side channel attacks over the network~\cite{Tsai19-Security}.
%when shared across side channel attacks~\cite{Meltdown,Spectre}

\stepcounter{reqs}
\boldpara{R\arabic{reqs}: Extendable.}
With the fast development of datacenter applications, hardware, and network, a good memory disaggregation solution should be flexible and extendable,
for example, to support more advanced APIs like pointer chasing~\cite{StRoM,AIFM},
to offload some application logic to memory devices~\cite{AIFM,XXX},
or to plug different network transports~\cite{Homa,NDP,pFabric,XXX} and congestion control algorithms~\cite{Swift,XXX}.

%\stepcounter{reqs}
%\boldpara{R\arabic{reqs}: Easy and cheap to deploy.}
%opportunity
%asymetric
%application aware of disaggregated memory

\input{fig-architecture}

\subsection{Physical Disaggregated Memory}
\label{sec:pdm}

One way to build disaggregated memory is to treat it as raw, physical memory, 
\ie, client servers send read/write request with physical memory address, and the memory node directly read/write to that address without any address mapping.
We call this model {\em \pdm}.
The \pdm\ model has been adopted by a set of non-RDMA interconnect proposals~\cite{Genz-citation,CXL-citation,CCIX,OpenCAPI}
and two RDMA-based software systems~\cite{Tsai17-SOSP,Tsai20-ATC} 
(these systems use the OS kernel to register physical memory directly, which is a special RDMA configuration mechanism).
In order to not allow applications accessing raw physical memory (which has security, issues),
these solutions add an indirection layer (either in hardware~\cite{Genz-citation,CXL-citation} or software~\cite{Tsai17-SOSP,Tsai20-ATC})
at the client side to map client process virtual addresses~\cite{Genz-citation,CXL-citation,CCIX,OpenCAPI} or client objects~\cite{Tsai17-SOSP}/keys~\cite{Tsai20-ATC}
to physical memory addresses at the disaggregated memory nodes. 

There are several common problems with all the \pdm\ solutions.
First, \pdm\ requires the client side to manage disaggregated memory, which is much harder and performs worse than if management is done at the memory side.
For example, client servers need to coordinate with each other or use a global controller~\cite{Tsai20-ATC} to perform tasks like memory allocation,
and when some memory needs to be migrated from one memory node to another (\eg, because of load balancing), 
all client servers  that have mapped this memory need to update their mappings.
Such complex client-side memory management defeats the purpose and benefits of disaggregation (\textbf{R5}).
Second, exposing physical memory creates potential security issues (\textbf{R6}).
Memory nodes have to trust that all client servers will send proper requests only to their allocated physical memory portion. 
%coordination across client servers (\eg, through a global controller~\cite{Tsai20-ATC} or a distributed consensus system).
Finally, all existing \pdm\ solutions require physical memory pinning at memory nodes, causing memory wastes (\S\ref{sec:pagefault}).
%it is also unclear how page faults will be handled.

In addition to the above common problems, none of the non-RDMA interconnects have been actually built (when they do, 
they will require new hardware at compute servers and switches in addition to memory nodes), 
and these fabrics provide coherence across different endpoints, which is costly and not always necessary.

%Recently, new cache-coherent interconnects like Gen-Z~\cite{Genz-citation} and CXL~\cite{CXL-citation}
%have been proposed to connect heterogeneous components in a rack~\cite{Genz-citation,CXL-v2} or in a server~\cite{CXL-citation,CCIX,OpenCAPI}.
%for single-machine or rack scale memory accesses.
%They usually expose a global memory space (that covers memory and accelerator memory) to applications running at the compute (client) 
%side and guarantee cache coherence among different compute and memory components.



\subsection{Virtualized Disaggregated Memory}
\label{sec:vdm}

The reason behind the \pdm\ model's issues is its physical abstraction of disaggregated memory.
Thus, we believe that disaggregate memory should expose a \textit{virtualized} memory abstraction,
and memory management and address mapping should happen at the memory pool, not the compute pool (client servers).
By hiding the physical nature of disaggregated memory under a virtual abstraction,
disaggregated memory can have the same benefits as what traditional virtual memory system provide, 
such as on-demand allocation (paging) and protected accesses across different applications.
By performing memory management at the memory node, we can avoid orchestration across client servers
and transparently perform tasks like replication and migration.
Both \sys\ and RDMA offer a virtualized disaggregated (remote) memory abstraction.
However, the virtualized view of them are completely different, and as we will show next, RDMA has many issues when used for memory disaggregation.
%As we will show shortly, RDMA cannot meet these requirements and is an ill fit for memory disaggregation.



\if 0

%This section discusses related topics 
%and motivates our work. %existing proposals and attempts to build remote memory
%and motivates programmable hardware-based disaggregated memory.
%We also cover related works in this section.

\subsection{Non-Disaggregated Remote Memory}
\label{sec:remotemem}

The idea of using non-local machine's memory dates back to the early 90s when research in 
distributed shared memory (DSM)~\cite{Shasta,Bennett90-PPOPP,Fleisch89-SOSP,Keleher92-ISCA} 
and distributed operating systems~\cite{Sprite88,Amoeba90} boomed.
Recent years have seen a rise of new interests in this idea because of datacenter network improvements~\cite{Aguilera17-SOCC}.
Several RDMA-based distributed memory systems have been proposed %in recent years
including Grappa~\cite{Nelson15-ATC}, FaRM~\cite{FaRM}, and Hotpot~\cite{Shan17-SOCC}.
%There are mainly two forms of using non-local (remote) machine's memory.
These systems use a machine's memory for both applications running locally and on remote machines.
Each machine manages its own memory and runs application processes.
Similar to traditional DSM systems, these systems require complex and costly consistency protocols for concurrent accesses.
Moreover, % important, %memory in these systems is not disaggregated 
they lack the benefits of disaggregation. % (see below).
%The second type reserves some memory space exclusively for remote accesses.
%To use these systems in a cluster setting, another distributed software system is usually needed on top of them.

\subsection{Resource Disaggregation}
\label{sec:disaggregation}

Resource disaggregation is a notion to separate different types of resources into different pools,
each of which can be independently managed and scaled.
Applications can allocate resources from any available node in a resource pool, resulting in tight resource packing. %regardless of where other types of resources sit.
Because of these benefits, % its manageability, independent scaling, and efficient resource utilization benefits,
many datacenters have adopted the idea of disaggregation, often at the storage 
layer~\cite{FACEBOOK-BRYCECANYON,FB1,SnowFlake-NSDI20,AMAZON-S3,AMAZON-EBS,Ali-SinglesDay}.
%layer~\cite{FACEBOOK-BRYCECANYON,FB1,SnowFlake-NSDI20,Decibel-NSDI17,AMAZON-S3,AMAZON-EBS,Klimovic18-ATC,RackScaleDisaggregation}.
%As a recent success story, Alibaba listed their storage disaggregation as one of the five reasons
%that enable them to serve the peak load of 544,000 orders per second on the 2019 Single's Day~\cite{Ali-SinglesDay}.

With the success of disaggregated storage and the fast developments in datacenter network speed,
researchers in both academia and industry started to seek ways to disaggregate memory 
(and persistent memory)~\cite{Lim09-disaggregate,FireBox-FASTKeynote,IntelRackScale,Lim12-HPCA,Shan18-OSDI,RAMCloud,Tsai20-ATC}.
Disaggregated memory proposals so far have taken two main approaches.
The first type treats the disaggregated memory layer as a {\em passive} party (raw, physical memory space with no processing power);
the compute pool manages the memory pool and provides high-level services to applications~\cite{HP-TheMachine,Tsai20-ATC,Lim09-disaggregate,Nitu18-EUROSYS}.
%that requires the compute pool for further management and high-level interface, 
The main problem of passive disaggregation is the excessive network RTTs needed when completely separating processing and memory.
% in passive disaggregated memory results in excessive RTTs and performance loss.

The second type (active disaggregated memory) organizes the disaggregated memory pool with regular servers and runs all or part of management software 
at these servers' CPUs~\cite{InfiniSwap,NAMDB,Kalia14-RDMAKV,Aguilera18-ATC}. 
%Recent proposals in this type include RDMA-based remote memory swap system~\cite{InfiniSwap}, remote database system~\cite{NAMDB}, 
%remote key-value store~\cite{Kalia14-RDMAKV}, and remote memory system with file interfaces~\cite{Aguilera18-ATC}.
%hey all run their memory systems on regular machines and use those machines' CPU to manage the memory spaces.
Co-locating management with memory reduces network RTTs.
However, these server-based solutions increase owning and energy cost, with full servers and large amounts of CPU cycles at the memory layer.
Moreover, the number of CPU cores limits the amount of parallel memory requests a memory server can handle.
An alternative way of building active disaggregated memory is to run management software in low-power cores.
However, recent work shows that low-power cores cannot meet the high-bandwidth and low-latency demands of memory systems~\cite{Tsai20-ATC}.

\phdm\ solves the problems of both these two existing disaggregated memory models.
By managing memory and providing distributed memory services in hardware at \MN{}s,
\phdm\ can achieve great performance, low network bandwidth consumption, and low monetary and energy cost.

LegoOS~\cite{Shan18-OSDI} is a distributed OS that takes a {\em partially} active disaggregation approach. 
%designed for resource disaggregation. %, which also advocates for managing resources at the resource nodes.
It runs a virtual memory system at its disaggregated memory pool and exposes a virtual memory interface to the compute pool.
%However, a virtual memory system is all what LegoOS' memory layer runs.
To support higher-level memory services, LegoOS still needs to add a software layer at the compute side.
More important, LegoOS has no real hardware design or implementation.
%runs all management in software on regular servers that are emulated as resource devices.
HPE's ``The Machine'' (Memory-Driven Computing) project~\cite{HP-TheMachine,THEMACHINE-HOTOS,HP-MODC-POSTER,THEMACHINE-WEB}
is another proposal that adopts the partially active disaggregation approach.
It separates a pool of DRAM/NVM from a pool of SoCs with a special interconnect inside a rack. % through a special interconnect~\cite{Genz-citation}. 
Memory instructions running at SoCs are transparently translated to access the DRAM/NVM pool,
and the translation is performed either at the interconnect~\cite{Genz-citation} or at the memory pool.
Similar to LegoOS, the Machine still needs extra software running at the SoC pool to provide high-level memory services.
Moreover, neither its design nor its maturity is known to the public.
%The DRAM/NVM pool provides a global memory address space,
%which requires extra software running at the SoC pool to manage and . % in, and use the memory pool.

\subsection{RDMA and Other Network Technologies}
\label{sec:rdma}

Datacenter network speed has increased dramatically in the past decade.
%Most datacenters now run on 10\Gbps/server or 40\Gbps/server networks~\cite{CatapultV1,Facebook-10GDatacenter},
%with 100\Gbps\ and 200\Gbps\ networks on the horizon~\cite{Facebook-100G,Mellanox200Gbps}.
%Meanwhile, network RTT can be as low as 1\mus\ for a single hop~\cite{Mellanox-Switch}.
High-bandwidth, low-latency networks give rise to a surge of interest in exploring remote or disaggregated 
resources~\cite{FaRM,FireBox-FASTKeynote,Shan18-OSDI,HP-TheMachine}.
%Network's much faster frequency speedup than CPU's~\cite{XXX} also motivated offloading various application and 
%I/O functionalities to hardware.
%Both these hardware trends are in line with what we propose in \phdm.

A high-speed network technology that several major datacenters have adopted~\cite{AZURE-RDMA,ALIBABA-RDMA} is
{\em Remote Direct Memory Access} (RDMA),
%RDMA supports both {\em one-sided} and {\em two-sided} communication to remote memory.
%One-sided RDMA allows one machine to directly read and write another machine's memory without involving the latter's CPU.
%Two-sided RDMA works like traditional messaging, involving both sender and receiver CPU.
which is the communication media adopted by most remote memory systems. % use RDMA as the communication media.
%with one-sided RDMA being used by systems where remote memory are managed by local (compute) machines~\cite{DPM}
%and two-sided RDMA used by systems where each machine manages its own memory~\cite{Kalia14-RDMAKV,Mitchell13-ATC}.
%With the help of one-sided RDMA and other one-sided network technologies~\cite{GenZ},
%several software systems have been proposed to treat 
%Albeit its superior performance, RDMA's limited interface is too restrictive for most applications,
Although several recent proposals of hardware~\cite{StRoM,Aguilera-FarMemory} and software~\cite{Tsai17-SOSP,HyperLoop} extensions to RDMA made it more flexible and performant, 
RDMA is still an ill fit for memory disaggregation.
The RDMA protocol and its implementation are both tightly bound with the processor that co-locates with the memory.
At least a process running on this processor needs to perform virtual memory allocation 
and registration through an OS and then share the allocated virtual memory addresses
with other (client) servers that wish to access the allocated memory. 
Essentially, RDMA's abstraction is a {\em host-server-centric} memory view.
What fits disaggregated memory and what \phdm\ provides is a {\em client-centric} memory view 
where client applications running on a server can directly access remote memory without the need to contact or maintain 
any additional processes or OSs running at the memory side.
Moreover, \phdm\ is a system-level design that has built-in distributed support, while RDMA is just a network layer that needs another software distributed system. 
%a client-side address space in \phdm\ could span multiple \MN{}s. %memory nodes.
%This client virtual address space can also span multiple \MN{}s.

Recently, new cache-coherent interconnects like Gen-Z~\cite{Genz-citation} and CXL~\cite{CXL-citation}
have been proposed for single-machine or rack scale memory accesses.
They expose a global memory space to applications running at the compute (client) 
side and guarantee cache coherence among applications and memory.
They are low-level, physical-layer solutions for accessing disaggregated memory.
With additional software systems, they could be used to build passive disaggregated memory.
\phdm's active disaggregated memory model saves network RTTs and client-side CPU cycles.
Moreover, the need to mainain cache coherence limits the scalability of these interconnects, and they require the replacement of existing datacenter network infrasturcture.
\phdm\ does not have cache-coherence scalability bottlenecks
and builds on Ethernet and can directly be deployed in today's datacenters.
%Rack-scale cache-coherent interconnects like CXL and Gen-Z provide a hardware layer to access disaggregated memory. 
%Software layer needs to be added on top (at the CPU side) to manage the disaggregated memory space.

\subsection{HADM Benefits and Use Cases}

The \phdm\ model offers several benefits over existing proposals. 
%that are key to meeting today's datacenter needs.
Unlike non-disaggregated remote memory, 
\phdm's separate, self-contained disaggregated memory layer is easy to configure, manage, and scale.
Compared to software-based approaches, 
\phdm\ can achieve 
%with hardware-based implementation, remote memory services can achieve
high-bandwidth, low-latency performance 
and sustain large concurrent loads
without paying the high costs of full servers.
Unlike passive disaggregated memory,
%By offering high-level distributed memory services, 
applications can build different remote memory services and/or offload
their near-data computation to the memory pool, 
improving performance and reducing CPU cycles.
%easily use remote memory without 
%worrying about its distributed nature or dealing with low-level interfaces.
%Finally, programmable hardware enables the reuse of the same hardware for different 
%types of memory services, yielding faster and cheaper deployment. %option than ASIC.

Many types of applications can make use of \phdm.
For example, applications or libraries can store large in-memory data structures 
like hash tables and tree indices at \phdm's memory pool and offload operations
like hash lookup and tree traversal to move computation closer to data.
More advanced types of application offloading are also possible, such as data 
processing and data analytics.
Applications can also use the memory layer of \phdm\ as a location to cache storage 
data or to share data across different compute nodes, 
\eg, storage-data caching or shared states for serverless computing systems.
Finally, OS and low-level systems software can build more functionalities like remote swap over \phdm\
and offer applications transparent accesses to remote memory.
See Appendix for further discussion.


\fi


\if 0
\sys\ is also different from previous computation offloading systems in terms of its hardware choice.
Previous solutions use either FPGA or ARM-based SoC to build their smart devices.
%with most of them also include a full NIC on board.
\MN{}s in \sys\ include both FPGA and ARM 
and use them for different planes. %, with the former used for the data plane and the latter used for the control plane.
%\sys\ integrates all the data path, including a lean network stack, on a single FPGA chip,
%while moving all the control plane and metadata operations to the SoC.
In doing so, \sys\ could achieve the best performance, cost, and programmability
combination that fits the need of a remote memory system.
%FPGA has seen an increasing adoption in industry~\cite{XXX} and more research interests~\cite{XXX} in recent years.
%Among the many FPGA-based systems, KV-Direct~\cite{KVDIRECT} and Catapult~\cite{XXX} are most relevant to \sys.
\fi

\if 0
Among all existing computation offloading solutions, three are the most relevant to \sys. 
KV-Direct~\cite{KVDIRECT} is a remote key-value store built on FPGA.
%Similar to \sys, it also integrates a lightweight network stack on the FPGA chip.
Unlike \sys, it targets a non-disaggregated environment and 
relies on the host CPU to perform metadata tasks such as memory allocation.
StRoM~\cite{StRoM} is a recent hardware proposal that includes a full RoCE (RDMA-over-Converged-Ethernet) network stack
and several high-level APIs like pointer chasing on an FPGA.
Although StRoM extends RDMA's restricted APIs to a more feature-rich interface,
it still has the same host-based memory view like RDMA (\S\ref{sec:rdma}).
Moreover, it has no distributed systems support.
Catapult~\cite{Catapult,CatapultV1} is a general-purpose distributed FPGA computation-offloading platform developed and deployed at Microsoft.
%which has been used for network-function offloading~\cite{AccelNet}, deep-learning inference~\cite{Brainwave}, and Bing search~\cite{CatapultV1}.
%Although Catapult is also a distributed FPGA-based platform, 
Different from \sys, Catapult is designed for a non-disaggregated environment 
and targets general computation offloading instead of memory management/services.
\fi


\if 0
Conceptually, the \phdm\ model could be built using any programmable hardware technologies.
For example, a SmartNIC could be extended to a programmable disaggregated memory device by attaching some memory chips to it.
Processor-based SmartNICs usually attach an ARM-based SoC or a small CPU to a NIC~\cite{BLUEFIELD,BROADCOM-SMARTNIC}.
Software can be easily deployed in the processor.
However, our experiments show that the processor cannot meet the performance requirements of high-speed network.
Hardware-based SmartNICs attach an FPGA chip to a NIC~\cite{INNOVA,SOLARFLARE-FPGA}.
\sys's hardware architecture is close to these SmartNICs, both using FPGA as programmable hardware (and thus could easily be modified to run on them).
Differently, \sys\ does not use a separate NIC and integrates the network stack with the memory services, 
saving both monetary cost and the performance overhead of communicating between two chips.
\fi



==> v1-rdma.tex <==
\section{RDMA Issues and \sys\ Solutions}

{\em Remote Direct Memory Access} (RDMA), a high-speed network technology that allows direct access to memory on a remote server,
has been adopted by several major datacenter\cite{AZURE-RDMA,ALIBABA-RDMA}.
It is also the communication media adopted by most existing remote and disaggregated memory systems~\cite{XXX}. 
However, as this section will present, RDMA --- its interface, memory system, and network protocol --- 
are all ill fits for memory disaggregation (esp. for virtualized disaggregated memory),
and existing workarounds all have their limitations.
\sys\ solves RDMA's issues by redesigning and co-design with the virtualized disaggregated memory model.
Figure~\ref{fig-arch} illustrates the architectural differences between RDMA and \sys.
%RDMA supports both {\em one-sided} and {\em two-sided} communication to remote memory.
%One-sided RDMA allows one machine to directly read and write another machine's memory without involving the latter's CPU.
%Two-sided RDMA works like traditional messaging, involving both sender and receiver CPU.
%with one-sided RDMA being used by systems where remote memory are managed by local (compute) machines~\cite{DPM}
%and two-sided RDMA used by systems where each machine manages its own memory~\cite{Kalia14-RDMAKV,Mitchell13-ATC}.
%With the help of one-sided RDMA and other one-sided network technologies~\cite{GenZ},
%several software systems have been proposed to treat 
%Albeit its superior performance, RDMA's limited interface is too restrictive for most applications,
%Although several recent proposals of hardware~\cite{StRoM,Aguilera-FarMemory} and software~\cite{Tsai17-SOSP,HyperLoop} extensions to RDMA made it more flexible and performant, 

%fine-grained sharing

\subsection{Memory System} 
\label{sec:memory}

\subsubsection{Memory Abstraction}
\label{sec:abstraction}
%\subsubsection{Tight Coupling to Co-Located CPU}

\boldpara{RDMA issue.}
Addressing of memory regions ({\em MR}s) registered with RNIC is through the virtual memory address space of a process running at the memory node
(the registering process, or {\em RP} in Figure~\ref{fig-arch}. 
Before registration, the RP first needs to allocate virtual memory address for the MR,
and after registration, the RP passes its virtual memory address and an \rkey\ assigned by the RNIC to application processes running at client nodes.
Essentially, RDMA's abstraction is not a {\em client-facing} one, creating two main issue.
First, clients need to communicate with the RP to allocate or use MRs, usually through a non-RDMA, out-of-band communication channel,
causing performance overhead.
Second and more severe for memory disaggregation, RDMA's abstraction implies that each memory node needs to have a co-located CPU that runs an RP.

\boldpara{Current solutions and their limitations.}
The current practice of using RDMA to access remote memory is to add a client-side software indirection layer 
to translate client application's view (\eg, process virtual memory addresses, object IDs) to MRs and RP's virtual addresses.
%to translate client application's view (\eg, process virtual memory addresses, object IDs) to MRs and RP's virtual addresses.
This approach involves two mappings: client address to RP virtual address (performed at client node) and RP virtual address to remote physical address (performed at memory node).
Doing so (unnecessarily) adds performance and memory space overhead.

\boldpara{\sys\ solution and benefits.}
\sys\ provides a {\em client-facing} virtual memory view 
where client application processes can directly access disaggregated memory with their virtual memory addresses.
\sys\ only performs one address mapping: application virtual address to remote physical address (done at memory node),
and \sys\ completely gets rid of the need for registering processes or server boxes at memory nodes.
Client applications can directly perform allocation, read, write, atomic APIs (\eg, \tas, \cas, \fence), 
and extended APIs like array indexing and pointer chasing (\S\ref{sec:extendability}) to disaggregated devices.

Note that the application ``virtual memory addresses'' \sys\ use (we call them \textit{\sys\ virtual memory address}es) may not necessarily come from normal process memory address space.
In fact, there are three ways to use \sys, and they have their own interpretation of what \sys\ virtual memory addresses mean,
as illustrated in Figure~\ref{fig-arch}.
First, an application process can explicitly call \sys\ APIs by linking to a \sys\ library which creates a special \textit{\sys\ virtual memory address space}
under the hood. 
The returned addresses of \alloc\ and input addresses of \sysread/\syswrite requests will all be virtual addresses in this space ({\em dvma-vaddr}).
Second, applications can sit on top a remote-memory swap system like FastSwap~\cite{FastSwap} and InfiniSwap~\cite{InfiniSwap},
which uses \sys\ virtual memory addresses as swap partition address ({\em swap-vaddr}) and performs \sys\ read/write to swap in/out disaggregated memory.
Third, a disaggregated compute device like pComponent in LegoOS~\cite{Shan18-OSDI} can integrate \sys\ into its hardware cache controller
and send \sys\ read/write with application processes' virtual addresses ({\em AP-vaddr}) for last-level-cache (called ExCache in LegoOS) misses. 

%Using client process virtual memory addresses also has the benefit that disaggregated memory can potentially be 
%integrated into client machine's memory microarchitecture~\cite{Lim09-disaggregate}.


\stepcounter{principle}
\ulinebfpara{Principle \arabic{principle}:}
\textit{The disaggregated memory abstraction should face client processes}.


\subsubsection{Memory Pinning and Page Faults}
\label{sec:pagefault}

\boldpara{RDMA Issue.}
Because RNICs rely on host machine's MMU and OS for virtual memory system support, they do not have any way to deal with page faults.
As a result, RDMA offers only two options, each having their own problem:
1) allocate and ping physical memory when registering MRs with RNIC, 
or 2) no allocation of physical memory and trap to the OS to handle page faults at first accesses.
Option 1) wastes physical memory space before they are used, 
while option 2) has poor performance for first accesses (and thus long tail latency) 
because of the costly communication between RNIC and the host OS (through interrupts)~\cite{ASPLOS17}.
Figure~\ref{fig-} \fixme{XXX}

\boldpara{Current solutions and their limitations.}
To not waste physical memory or causing high page fault performance overhead, 
one option is \textit{fine-grained pinning} where client application dynamically asks 
the memory process to register/unregister a new MR (and pin/unpin physical memory)  
immediately before and after the remote memory usages.
However, it is difficult to infer or ask programmers to specify first memory accesses, 
and RDMA's costly MR register operations significantly degrades application performance
(in our experiments, sending a network request and registering a new MR take \fixme{XXX} in total).
%Another solution proposed recently~\cite{ASPLOS-17} is to 
Thus, the common practice today~\cite{FastSwap,XXX} is to trade memory space for performancy by 
allocating a big MR and pinging its physical memory before an application starts.
%However, such \textit{coarse-grained pinning}'s resulting memory wastes would be a severe problem in a disaggregated setting, 
%as memory at  and should be used by applications as much as possible.

\boldpara{\sys\ solution and benefits.}
\sys\ completely eliminates pinning (and registering) with a virtual memory system that 
performs on-demand physical allocation and page fault handling --- just like what modern OS's provides,
but without the performance cost of RDMA's page fault mechanism.
The key to achieve this is our efficient implementation of the page fault handler in the memory device's main hardware pipeline.
Our main idea here is to move the slower, more complex, and non-deterministic allocation logic (both virtual and physical memory allocation)
to software running at a co-located low-power core, and to use an asynchronous methods to communicate 
between the software allocator and the hardware page fault handler.
With this novel virtual memory system design, our implementation has a \textbf{constant three-cycle latency of page fault handler}.
Figure~\ref{fig-} \fixme{XXX}
We will present the detailed design of our virtual memory system in \S\ref{sec:}.

\stepcounter{principle}
\ulinebfpara{Principle \arabic{principle}:}
\textit{Efficient space usage and performance can both be achieved by integrating virtual memory system in the hardware pipeline}.


\subsubsection{Memory Region}
\label{sec:mr}

\boldpara{RDMA issue.}
RDMA associates a set of metadata with each MR, namely an ID and two keys (\texttt{lkey} and \texttt{rkey}).
RNIC stores these MR metadata in its SRAM cache, and the memory consumption grows linearly with the number of MRs registered with the RNIC. 
When the SRAM is filled up, RNIC will swap the MR metadata to host memory (thrashing), causing significant performance degradation.
Figure~\ref{fig-} \fixme{XXX}

Another issue with MR is that RDMA uses it as the protection scope.
Thus, each client process needs to have at least one MR,
and if two client processes want to share some memory, the RP has to create a new MR.
In addition, metadata of different MRs share the same RNIC cache,
causing (remote) side channels that can be exploited to infer access patterns of victim clients~\cite{Tsai19-Security}.

\boldpara{Current solutions and their limitations.}
One way to reduce the number of MRs is to register a huge MR before an application starts and use a software layer to 
manange this MR (allocation) and map application memory areas to different parts of the MR.
However, as discussed in \S\ref{sec:pagefault}, huge MR will cause either memory waste or high tail latency (due to page faults),
and a new MR needs to be created for each protection scope.
LITE~\cite{Tsai17-SOSP} uses the OS kernel to register the entire server's physical memory as one MR when the system starts up
and to use a kernel module to allocate physical memory to applications.
LITE suffers from performance overhead of user-level-kernel crossings and all the drawbacks of the \pdm\ model (\S\ref{sec:pdm}).
1RMA~\cite{1RMA} uses a fix-sized region table

\boldpara{\sys\ solution and benefits.}
\sys\ gets rid of MR all together. 
With the per-client-process virtual memory space \sys\ offers, applications can allocate (and share) 
as many memory areas as they want without incuring any performance overhead.
%is all  with arbitrary memory areas in the space (through rmalloc instead of registering MR)
Figure~\ref{fig-} \fixme{XXX}

\stepcounter{principle}
\ulinebfpara{Principle \arabic{principle}:}
\textit{}.

\subsubsection{Page Table}
\label{sec:pte}

\boldpara{RDMA issue.}
RDMA uses page tables created and maintained by host CPU and OS to map MRs (RP virtual addresses) to physical memory.
To speed up page table lookup, RNIC caches hot PTEs (page table entries) in its SRAM.
Similar to the scalability problem of MRs, RDMA performance degrades significantly when cached PTEs fill up the SRAM.
Figure~\ref{fig-} \fixme{XXX}

\boldpara{Current solutions and their limitations.}
The common practice to mitigate RDMA's PTE scalability problem is to use huge pages (\eg, 2\GB),
which effectively reduces the number of PTEs~\cite{FaRM,Tsai17-SOSP,XXX}.
However, with large memory, even huge page PTEs could still fill up RNIC SRAM, 
and when it does, it could take up to four DRAM accesses from the RNIC (over PCIe) to walk a x86 page table and fetch a PTE.

\boldpara{\sys\ solution and benefits.}
We propose a new {\em overflow-free} hash-based page table design that bounds the size of PTEs to physical memory size 
and address translation to at most one DRAM access.
Specifically, we store {\em all} PTEs (from all client processes) in a hash table 
whose size is fixed and proportional to the physical memory size of a disaggregated memory device,
\ie, the hash table has enough entries to cover the entire physical memory (\eg, \fixme{XXX \MB\ for 100\GB\ physical memory and XXX page size}).
The hash value of a virtual memory address and its PID is used as the index to determine which hash bucket in the table the corresponding PTE goes to.
To lookup the page table, we always fetch
% compute its hash value (using the {\em lookup3}~\cite{lookup3-wiki} hash function) 
the entire bucket (with all its slots), in a single DRAM read.

Normally, a hash table with fixed slots will have an overflow problem because of hash conflicts.
We use a novel technique to {\em proactively avoid} hash overflows at virtual address allocation time.
To allocate a new virtual memory page, we keep trying available virtual memory addresses until there is one 
whose hash value would go to a bucket that still has an empty slot.
This allocation process is carried out in software running on an ARM core, while the page table lookup is performed by the hardware pipeline of a \sys\ device.
We trade potential retry overhead at allocation time for better run-time performance and simpler hardware design.
% core-memory implementation.
This overhead is manageable because 1) each retry is fast with our implementation~\cite{sec:metadataplane}, 
2) we employ huge pages, which means fewer pages need to be allocated, 
3) we choose a hash function that has very low collision rate~\cite{lookup3-wiki},
and 4) the \sys\ 64-bit virtual address space is huge.

Figure~\ref{fig-} \fixme{XXX}

\stepcounter{principle}
\ulinebfpara{Principle \arabic{principle}:}
\textit{}.

\subsection{Network System}
\label{sec:network}

\subsubsection{Connection, Reliability, and Ordering}

\boldpara{RDMA issue.}
RDMA's RC (reliable connection) mode, the only mode that supports both RDMA one-sided read and write operations,
is connection-oriented, requiring QPs (send\&receive queue pairs) to be established 
between a sender and a receiver before communication can happen.
RDMA implements its transport layer in hardware (RNIC),
and a reliable transport requires per-connection states.
Like MR and PTE, these states and other QP metadata are stored in RNIC SRAM, 
and QPs, too, have scalability issues.
Figure~\ref{fig-} \fixme{XXX}

\boldpara{Current solutions and their limitations}
A common mitigations to the QP scalability issue is QP sharing, 
where multiple threads in a workload or multiple workloads share a QP~\cite{FaSST}.
However, threads sharing a QP content for locks to use the QP,
and the FIFO order enforced by a QP can cause ``false ordering'' among workloads~\cite{1RMA}.
An alternative method is to use RDMA UD (unreliable datagram) mode.
The main issues with UD are its unreliable communication and 
its only support of two-sided RDMA, which requires the receiving node's CPU to be involved in the communication and thus does not fit the disaggregated memory model.

1RMA~\cite{1RMA} proposed a connection-less approach to perform remote read/write
and to use the reply of read/write requests as the ACK.
It relies on 

\boldpara{\sys\ solution and benefits.}
\if 0
Our insight is that we {\em can} achieve reliability without the need for connection or {\em any} states at the memory devices
by exploiting the {\em asymmetric} nature of memory disaggregation.
Our main idea is to shift all reliability tasks at the client side in software
and only include L1 and L2 in hardware (regular Ethernet NIC at client servers and a standard Ethernet MAC module at memory device hardware).
%and perform {\em all} reliable transport operations at the client side in software (\syslib).

Since all \sys\ operations are in the RPC style initiated by client servers, \ie, sending read/write requests and getting data/response back,
we use the reply as the ACK and matches replies to their corresponding requests using a request ID that is embedded in the packet header.
Each request's packet headers also include sender-receiver addresses, which will be used to construct reply packets. 
With these mechanisms, we essentially have a (unreliable) connectionless transport.
Below, we explain how we add reliability.

Network errors can happen when a packet is corrupted, loss, or reordered.
We use link-/physical-layer error correction like Forward Error Correction and retries that are already available in InfiniBand~\cite{MellanoxOFED} \fixme{and Ethernet???}
to deal with packet corruption, similar to prior practices~\cite{RAIL-NSDI17,FaSST}.
As the link layer does not (\fixme{or rarely?}) drop packets, packet loss is mainly due to buffer overflows in the network.
We control (minimize) packet loss with our client-side, software congestion/flow control mechanism (\S\ref{sec:cc}).
In the rare case of packet loss (either in a \sys\ request or its response), the client-side \syslib\ will fail after a request timeout
and retry the entire \sys\ request.
This leaves us with packet reordering, which is rare in non-multi-path network, but can still happen.

We take three approaches in handling packet reordering.
First, we guarantee that each request/reply is always delivered to upper layers in its entirety 
even when it is split into multiple link-layer packets that can be reordered.
We achieve this simply by using intra-request/reply sequence IDs to mark the proper ordering of packets 
and if needed, reorder them before delivering the request/reply.
Second, we offer synchronous APIs, with which we can guarantee that requests in the same session\footnote{Session is a \sys\ notion of }
is executed one after another. 
Thus, even without ordering guarantees from the network layer, synchronous requests will still be executed in order.
Finally, to offer more aggressive performance optimization, we offer asynchronous APIs, 
where multiple requests can be sent out before their replies are received.
Unlike synchronous requests, network reordering can affect asynchrnous requests' ordering.
We handle asynchronous requests' ordering in \sys\ with two methods:
1) the \syslib\ tracks read-write and write-write dependencies (outstanding read and write requests to the same address)
and issue dependent requests in a synchronous way;
2) we· offer a \fence\ operation, which lets a client process to wait until all outstanding asynchrnous requests have finished.
With these mechanisms, applications can achieve {\em release consistency}.

As a result, \sys\ memory devices completely remove the need for network states and thus all network-related scalability bottlenecks,
and client servers only need regular L2 Ethernet NICs with no NIC scalability issues either.
Figure~\ref{fig-} \fixme{XXX}

\stepcounter{principle}
\ulinebfpara{Principle \arabic{principle}:}
\textit{Efficient end-to-end reliability and stateless memory devices can be and is better achieved by shifting reliability handling to client-side software.}
%with unreliable, connectionless network
%Relaxing strict network reliability and handling reliability at system/application level }.  

\subsubsection{Congestion and Flow Control}
\label{sec:cc}

\boldpara{Issue}
RDMA over Converged Ethernet (RoCE) relies on link-layer Priority Flow Control (PFC~\cite{PFC}) to provide a drop-free substrate.
PFC is a mechanism for switches and NICs to avoid buffer overflow by forcing the immediate upstream entity to pause (through PFC pause frames).
However, PFC has a well-known head-of-line blocking issue and a risk of deadlock that make it infeasible to deploy at large scale~\cite{Zhu15-SIGCOMM}.

\boldpara{Current solutions and their limitations}
A common practice adopted by datacenters is to reduce PFC triggering by adding hardware-based congestion control schemes~\cite{Zhu15-SIGCOMM,hpcc-sigcomm19}
or by switching to a backup TCP network~\cite{RDMA-NSDI21}.
These schemes do not fit our needs, as we 
Recently, 1RMA~\cite{1RMA} proposed to 
two RTT writes

\boldpara{\sys\ solution and benefits.}
RDMA's network protocol treats all endpoints the same, \ie, a symmetric protocol.
We make two insights here.
First, with our design and implementation, a \sys\ memory device' internal throughput is always higher than its port bandwidth.
Thus, there will be no buffer overflow in a \sys\ memory device (\ie, it is faster than the network), 
and there is no memory-side in-cast problem and no need for memory-side flow control.
Second, 
client-side controlled congestion control
reactive, delay-based, window based 
solicitation window for client-side incast

\stepcounter{principle}
\ulinebfpara{Principle \arabic{principle}:}
\textit{}.

\subsection{Extendability}
\label{sec:extendability}

\boldpara{Issue}
limited primitives
bundled network stack and memory system, in a closed system
As a result, datacenters cannot easily deploy new transports~\cite{Homa,NDP,pHost} or congestion-control algorithms~\cite{1RMA,XXX}.

\boldpara{Current solutions and their limitations}

\boldpara{\sys\ solution and benefits.}
\sys\ allows \textit{easy extension} to different network stacks, high-level APIs, and to distributed disaggregated memory
modularized approach, each could be replaced by a new one

\stepcounter{principle}
\ulinebfpara{Principle \arabic{principle}:}
\textit{}.

\subsection{Putting It Together}


==> v1-tbl-system-cmp.tex <==
{
\begin{table*}[th]
\footnotesize
\begin{center}
\begin{tabular}{ $l!{\vrule width 1.6pt} ^c | ^c | ^c!{\vrule width 1.2pt} ^c | ^c | ^c | ^c}
System & Addressing & Mapping Location &  Page Fault &  Tail Latency & Scalability Bottlenecks &  Management &  Extendability \\
\hline
\ChangeRT{1pt}
RDMA   		& Memory virtual& Client\&Memory & Int host OS	& High	& Conn, MR, PTE	& Hard   & Poor \\
\pdm\   	& Physical	& Client & No/Unknown	& 	&	& Hard   & Poor \\
\rowstyle{\bfseries}
\sys\ 		& Client virtual& Memory & In hardware 	& Low	& None	& Easy   & Good 
\end{tabular}
\end{center}
\vspace{-0.15in}
\mycaption{tbl-system-cmp}{Comparison of RDMA, \pdm, and \sys.}
{
}
%\vspace{-0.1in}
\end{table*}
}



==> v2-intro.tex <==
\section{Introduction}
\label{sec:introduction}

Modern data-center applications like graph computing, data analytics, and deep learning have increasing demand for access to large amounts of memory~\cite{XXX}.
Unfortunately, servers are facing {\em memory capacity walls} because of pin, space, and power limitations~\cite{HP-MemoryEvol,ITRS14,MemoryWall95}.
Going forward, it is imperative for datacenters to seek solutions that can go beyond what a (local) machine can offer, \ie, using remote memory.
At the same time, data centers are seeing the needs\cite{Ali-SinglesDay,SnowFlake-NSDI20,FB1} from management and resource utilization perspectives
to {\em disaggregate} resources --- separating hardware resources into different network-attached pools 
that can be scaled and managed independently.
These real needs have pushed the idea of memory disaggregation:
organizing computation and memory resources as two separate network-attached
%segregating memory from computation into a network-attached pool
%Memory disaggregation is thus an appealing proposal that has gained a lot of traction recently. 
%Memory disaggregation segregates memory from compute over the network 
pools: compute nodes ({\em CN}s) and memory nodes ({\em MN}s).
%\footnote{We call the resulting compute node {\em \CN} and the memory node {\em \MN}.
%\CN{}s and \MN{}s can both be regular servers or network-attached compute/memory devices.}.

Unlike the traditional computer system where memory is virtualized, managed, and used all at the same server, % at the server CPU and MMU,
memory disaggregation poses new design questions on
\textbf{Q1)} \textit{what abstraction disaggregated memory exposes},
\textbf{Q2)} \textit{where memory management happens},
%\textbf{Q2)} \textit{where memory management and address translation happen},
%Q3) where memory address translation is performed, % (\CN, \MN, or both?), %(address translation, allocation)
%Q3) whether and where virtual memory system (\eg, on-demand allocation) is implemented,
\textbf{Q3)} \textit{how to build \MN{}s?}, 
%\textbf{Q3)} \textit{what type of virtual memory system to build},
\textbf{Q4)} \textit{how to perform network communication between \CN{}s and \MN{}s},
and \textbf{Q5)} \textit{how to build applications when memory is far from computation}.
%\textit{where computation happens}. % (\CN, \MN, or both?),
%where should network management happen
%and Q4) what goes into software and into hardware.
%The decisions of these design choices
%will guide both the underlying system design and the application usage models of disaggregated memory.
We believe that each of the above questions demands a new examination, % that is guided by 
as memory disaggregation poses new requirements in usage model, performance, cost, and operation complexity.
%new requirements of memory disaggregation in performance, cost, and operation complexity.
Below are our four key insights that motivate and guide this work.
%Memory disaggregation presents new requirements in performance, cost
%Existing approaches in building disaggregated-memory systems take three main forms,
%and they have different choices of the above questions and their own limitations.

First, disaggregated memory should expose an abstraction that is versatile
enough to support many different uses.
One such abstraction is {\em per-client virtual memory},
where each client has an isolated space that it can access with virtual memory addresses at byte granularity
%just like how traditional process address space works
 (\textbf{Q1}).
Just like the classical virtual memory abstraction, this abstraction is low-level and generic enough to support many applications
and high-level enough to protect and hide raw memory. 
%This abstraction inherits the versatility and transparency benefits of the classical virtual memory abstraction. %process address spaces:
%1) application-level programs and low-level systems like databases and JVM can all sit on the same abstraction
%with each of them properly isolated,
%and 2) the physical location of disaggregated memory can be transparent and thus non-contiguous and moved around.
Behind this abstraction,  
memory management (and as a result, address translation) should happen at {\em where the memory is}, \ie, at \MN{}s (\textbf{Q2}).
%and mapping of this virtual memory to \MN's physical memory should happen at \MN{}s (Q2).
%A client-facing virtual memory abstraction will Each client process should have their own protection domain
This is because 1) by encapsulating management in the disaggregated memory pool and allowing client applications to 
access it as a black box, %behind the familiar, native virtual memory interface, 
we can achieve independent, transparent resource pool management,
which is a key reason behind industry's wide adoption of storage disaggregation~\cite{FACEBOOK-BRYCECANYON,FB1,SnowFlake-NSDI20,Ali-SinglesDay}; %why storage disaggregation has become the recent industry norm;
and 2) performing management at one location (\MN) can avoid the synchronization overhead of a dispersed management mechanism.
However, most existing systems either treat disaggregated memory as raw, physical memory 
and manage it at \CN{}s~\cite{Genz-citation,CXL-citation,CCIX,OpenCAPI,Tsai20-ATC} or 
split memory management and address mapping across \CN{}s and \MN{}s~\cite{InfiniSwap,FastSwap,Semeru,AIFM} (Figure~\ref{ref-arch}).
%first map application interface to an intermediate abstraction at \CN{}s and then map the intermediate
%abstraction to physical memory at \MN{}s~\cite{InfiniSwap,FastSwap,Semeru,AIFM}.
%The former 

Second, we should build \MN{}s as standalone hardware devices without a server box (\textbf{Q3}),
%as the potential cost-saving, performance-improvement, and scalability
as its benefits outweigh the complexity of hardware development.
Building \MN\ as a single hardware device avoids the monetary cost of a whole server box and the energy cost of a CPU.
It also avoids the performance overhead of NIC talking to the host server for handling disaggregated memory requests.
%Hardware can also have greater parallelism than 
Today's disaggregated memory systems unfortunately have a strong reliance on host CPU, MMU, and OS
for running a virtual memory system, even though these systems themselves do not necessarily need to run anything at the host server.
The solution is obvious but never carried out before: building the virtual memory system in \MN\ hardware.


\if 0
Second, to virtualize and manage memory, \MN{}s should build a virtual memory system with on-demand allocation,
and do so in a performance- and cost-efficient way (\textbf{Q3}).
The classic wisdom of %allocating virtual memory addresses when applications explicitly request memory allocation and 
delaying the allocation of physical memory to application access time
has shown to be the most efficient way of utilizing memory space.
%Unfortunately, no existing disaggregated memory systems address this problem;
However, most existing disaggregated and remote memory systems allocate and pin all memory up front (\ie, no on-demand allocation)~\cite{FaRM,XXX},
because the only other option of NIC interrupting the host CPU (OS) to handle page faults is too slow.
% (which wastes memory) or
%rely on a host CPU and OS to handle page faults~\cite{XXX}
%hand over the virtual memory tasks completely to the host CPU/OS 
%(which not only adds high CPU energy and cost to \MN{}s 
%but also results in significant performance overhead when communicating between the NIC and the CPU for tasks like page fault handling).
%adopt what has withstood the test of time
%and worked well for a sea of applications: 
%a page-based virtual memory system with on-demand allocation (\textbf{Q3}).
%This fine-grained, just-in-time allocation is the most efficient way to utilize memory space
%and the most flexible way to enforce memory protection and sharing.
%Unlike segmentation~\cite{1RMA}, page 
To minimize both memory waste and performance overhead, we should support on-demand allocation
%an on-demand virtual memory system should be implemented 
in the same hardware that receives and processes client network requests.
%and the resulting \MN{} should be a stand-alone network-attached device.
%Although the on-demand virtual memory model has been well understood and standardized in modern computers' CPU, MMU, and OS chain,
%memory disaggregation presents an interesting new challenge:
%\textit{is it possible to implement a virtual memory system in hardware} so that \MN{}s can be cheaply built and run without a server box?
%reliance on host CPU, MMU, OS to implement 
%cost to interrupt CPU to handle page faults
%As a result, in practice, all disaggregated memory system pin memory up front
%the lack of on-demand allocation causes 
\fi

Third, we can improve communication performance and reduce cost by 
exploiting the unique nature of memory disaggregation to co-design the network layer
%without changing existing datacenter network infrastructure 
(\textbf{Q4}).
Unfortunately, existing disaggregated memory systems lose this optimization opportunity by sitting on RDMA or TCP.
%Not designed for memory disaggregation, 
RDMA and TCP have two fundamental features that make them unfit for memory disaggregation:
1) they have the same design for all endpoints (\ie, symmetric),
while memory disaggregation are asymmetric in nature (\CN{}s are always the request initiator and \MN{}s only respond to requests);
2) their reliable transports are connection-based and follow strict packet ordering.
These features result in scalability bottlenecks and added hardware complexity.
However, as we will show in \S\ref{sec:network}, neither are required if we can customize the network layer for the client-facing virtual memory model.

% should be aware of and customized for disaggregated memory and the client-facing virtual memory abstraction,
%and do so without changing existing datacenter network infrastructure (\textbf{Q4}).
%All existing disaggregated memory systems sit on RDMA or TCP.
%Both of  which are an ill fit for memory disaggregation (\S\ref{}).
%Although improvements to RDMA~\cite{1RMA} have been proposed, 
%they often require network infrastructure changes and are not designed for memory disaggregation.

%Finally, applications should be able to easily choose how to split their computation across \CN\ and \MN\ 
%(from all at \CN\ to all at \MN), as some types of computation are better performed close to data and 
%other types are better done at (\textbf{Q5}).
Finally, in order to reduce the network communication between \CN{}s and \MN{}s,
applications should be able to easily and safely offload their less computation-intensive tasks to \MN{}s (\textbf{Q5}).
%one way to avoid the network communication to disaggregated memory is to move computation to memory.
%a disaggregated memory system should allow applications to easily and safely offload their less computation-intensive 
%processing to \MN{}, while keeping their computation-intensive tasks at \CN{}s (\textbf{Q5}).
%Offloading also allow \CN{}s to dedicate its (more powerful) computation resources to complex application execution.
%Processing data at memory can avoid network round trips and bandwidth consumption of moving data to \CN{}s for computation.
%(\eg, performing SQL SELECT at \MN{}s before sending the filtered data to \CN{}s for further processing).
%Having realized this critical performance need, more disaggregated systems have added the support for computation offloading,
%Most existing disaggregated memory systems either do not support computation offloading or offload computation
%as software running at \MN\ server CPU~\cite{AIFM,XXX}.
%CPU-based offloading incurs high energy costs, % compared to non-disaggregated systems.
%, with full servers and large amounts of CPU cycles at the memory layer.
%and the number of CPU cores limits the amount of parallel memory requests an \MN\ can handle.
%Moreover, there lacks a coherent 
%In comparison, 
%Offloaded computation can execute as software in a CPU at \MN~\cite{AIFM,XXX}.
%Compared to software-based computation offloading~\cite{AIFM,XXX},
%While software is easy to implement, 
Furthermore, running offloaded computation in hardware is a desired option, %reduces \MN{}'s energy cost 
as it could achieve more parallelism and performance customization,
while avoiding CPU energy cost.
%It also fits the desired goal of building \MN{}s without a CPU or a server box.
However, %a major obstacle of hardware-based offloading currently is 
%there is no good system support for offloaded computation to 
it is hard to offload computation to \MN\ hardware today,
largely because there is no good system support for offloads to use (virtualized) memory
and offloads running at \MN{}s cannot have a coherent memory view with computation running at \CN{}s.
%a lack of a coherent view across computation at \CN{}s and at \MN{}s.
%allow us to achieve the amount of parallelism that can match high-speed network line rate.
%However, a major challenge is the difficulty of programming and running applications on raw hardware,
%which is largely due to the lack of system support.

Based on these insights, we propose \textit{\sys} (\textit{Disaggregated Virtual Memory Access}), 
a cross-layer, software/hardware-codesign solution that %centers around 
allows both applications running at \CN{}s and computation offloads running at \MN\ hardware
to access \MN\ memory through a virtual memory interface.
%to have efficient virtual memory accesses to 
%offers efficient virtual disaggregated memory accesses to both application running at \CN{}s 
%and computation offloads running at \MN\ hardware.
\sys\ includes a memory system, a network system, and a framework for computation offloading,
all of which are catered towards the hardware-based disaggregated virtual memory model and memory disaggregation's unique requirements.
The \sys\ \MN\ is a new hardware device (\textit{\sysboard}) that we designed from scratch and prototyped with FPGA. %a Xilinx FPGA-based MPSoC board.
The rest of \sys\ uses common hardware and network infrastructure available in today's data centers with a user-space library (\textit{\syslib}) at each \CN,
making \sys\ easy to be adopted.

\sys\ offers three ways of using disaggregated memory.
First, applications or a system layer (\eg, a swap system~\cite{InfiniSwap,FastSwap}) running at \CN{}s can allocate (remote) virtual memory spaces and read/write data in them.
In addition, \sys\ offers a set of extended APIs like synchronization primitives and pointer chasing, % for applications running at \CN{}s to use,
and users can also write and deploy new extended APIs at \MN{}s.
Second, applications can offload some of their computation to \MN{}s.
\sys\ provides such offloads with the same virtual memory address space and interface as their \CN\ counterparts.
Finally, users can build \textit{memory services} that run entirely at \MN{} hardware (\eg, a key-value store).
\sys\ offers each memory service its own virtual memory address space.

\if 0
%\sys\ meets all the four memory disaggregation requirements and the following key goals:
%We design philosophies to achieve 
\sys's design emphasizes on several fronts:
\textbf{1) \textit{scalability}} --- we remove {\em all} scalability bottlenecks at \MN's network stack and request processing, 
giving \sys\ unlimited\footnote{as long as sustainable by port link bandwidth and total physical \MN\ memory size}
scale on the data path to the number of \CN{}s, client processes, and disjoint memory regions, 
\textbf{2) \textit{low tail latency and high throughput}} --- \sys's data path has bounded, predictable 
latency%\footnote{XXX\mus\ end-to-end read/write latency for access patterns} 
and can always achieve network line rate\footnote{100\Gbps\ with our FPGA prototype},
\textbf{3) \textit{low cost}} --- \sys\ completely removes the need for a server box and power-hunger CPUs at \MN{}s,
and we make \MN's data path {\em stateless} so that \sysboard\ can be built with small on-chip memory and simple logic, 
\textbf{4) \textit{unified system support for computation offloading}} --- 
\sys\ provides a framework that enables easier development and safer execution of computation offloads in hardware
and a unified virtual memory system support for computation running at \CN{}s and at \MN{}s applications,
and \textbf{5) \textit{extendible}} --- we take a modularized approach in building \sys\ and bake only minimal logic into fixed hardware,
allowing \sys\ to be easily extended and reconfigured.
\fi

%\if 0
\sys\ achieves 
\textbf{1) \textit{low tail latency and high throughput}} --- \sys\ achieves network line rate (100\Gbps\ with our FPGA prototype)
and low average and tail latency (\eg, 2.5\mus\ min and 2.7\mus\ max 16\,B read latency), 
\textbf{2) \textit{excellent scalability}} --- \MN{}s can freely\footnote{as long as sustainable by port link bandwidth and total physical \MN\ memory size}
scale with the number of \CN{}s, client processes, and disjoint memory regions,
\textbf{3) \textit{low cost}} --- \sys\ completely removes the need for a server box and power-hungry CPUs at \MN{}s,
%and \sysboard\ can be built with XXX\MB\ on-chip memory and simple logic,
\textbf{4) \textit{safe and flexible computation offloading}} --- 
applications can safely offload their computation and enjoy a unified virtual memory system support,
and \textbf{5) \textit{extendible}} --- existing application-level~\cite{AIFM} and system-level~\cite{InfiniSwap,FastSwap,Semeru} 
disaggregated memory solutions can easily use \sys\ as the low-level platform,
and \sys\ itself can be easily extended and reconfigured.
Achieving these goals requires novel design and careful engineering in almost every part of the system.
%Even with our four insights (which tell us what to build but not how),
%it is extremely challenging to achieve the above goals.

\if 0
The first challenge is to build a hardware-based virtual memory system that can deliver bounded data-path latency.
which 

Second, \textit{how to give \sysboard\ ``unlimited'' scalability without requiring }
stateless, bufferless, connectionless, no per client-process state (page table)

is it possible to achieve bounded data-path performance (low tail latency)
hash page table

\fi

%Our four insights presents what to build in a disaggregated memory system, but not how to build it. %so as to 
%There are achieve key goals that will make a disaggregated memory system successful.
%These goals include 
%
%Even with our insights, building the \sys\ system presents many demanding challenges,
%as 
%Building a disaggregated memory system that meets the
%Even with our insights as the overall guidance, meeting the above goals is extremely challenging,
%as 

The first major challenge is to build a full-fledged hardware-based virtual memory system that can deliver bounded, low latency for any type of data accesses.
%Today's software-based virtual memory system has long tails for page faults
Directly porting today's software-based virtual memory system to hardware will not only require huge hardware resources but also results in long tails for tasks like page fault handling.
%including address translation, virtual and physical memory allocation, and page fault handling.
%The main challenge here is to efficiently offload the virtual memory system to the device to achieve ``hardware'' performance without the development and monetary cost
%of building complex virtual memory logic in hardware.
%The first technical hurdle lies in building an on-demand virtual memory system in hardware that can achieve
%low tail latency and the throughput of network line rate, both of which are .
Our idea is to implement a {\em deterministic} hardware pipeline that bounds the latency of {\em all} memory access operations %including page fault handling 
%in a {\em deterministic} hardware pipeline 
%with guaranteed 
%{\em performance determinism} and to move metadata operations and 
and to keep non-deterministic and/or complex operations in software (running at few low-power cores in \sysboard).
We use a novel, asynchronous approach to efficiently interact between hardware and software to achieve good foreground performance.
%so that even when an operation requires results from slower and non-deterministic software, 
%its application-perceived foreground performance is still as fast as the hardware pipeline.
We further propose a new conflict-free hash-based page table design that bounds address mapping to take at most one memory access.
%The resulting \sys\ memory system finishes all memory read/write operations within three cycles and at most two memory accesses,
%even under page faults and under various scaling dimensions.

Another big challenge is to achieve near-unlimited scalability with only minimal hardware resources at \sysboard.
Our general idea is to avoid maintaining states or data structures that could grow with clients or \CN{}s.
For example, for \sys's memory system, we design the page table to have a total size proportional to the physical memory size on an \MN, 
not to the number of client processes using the \MN.
%and we avoid storing any per-client states at \MN{}s.
Similarly, we avoid maintaining any states that could grow with flows or clients at \sysboard.
%The challenge is to deliver end-to-end reliability while avoiding \MN-side states.
%completely {\em stateless} and {\em bufferless},
%which is more challenging than making \sys's memory system stateless, 
%as traditional connection-based, reliable network layers like RDMA and TCP are stateful and require packet buffer for retransmission.
%\sys's network system includes a connectionless transport and purely-client-managed congestion and flow control.
%Our key observation here is that client nodes and memory devices should be treated as different parties, 
%with the former always being the (active) request initiator and the latter being the (passive) responder.
To achieve this while delivering end-to-end reliability, 
\sys\ 1) uses a connection-less, RPC-like interface, % on top of a standard Ethernet link layer,
2) treats network errors as \sys\ request failure and re-executes the entire request, 
3) shifts stateful tasks like re-execution, packet ordering, and congestion control to the \CN\ side, % (in \syslib\ software),
and 4) removes ordering guarantees from the network and provides memory operation ordering at \syslib.
%Thus, we propose an asymmetric network protocol where the \MN\ side is completely 
%{\em stateless} and {\em bufferless} (so as to make \sysboard\ low cost and scalable),
%We shift all stateful operations like congestion control to the \CN\ side and to software.
%and the \CN\ side handles network states, packet ordering, and congestion/incast,
%all in software and in a way that is customized to memory disaggregation.
%Furthermore, user-controlled relaxed ordering 

%On top of the basic virtual memory interface, \sys\ offers a set of extended APIs such as pointer chasing
%and a framework for applications to easily offload their computation to \MN\ hardware.
% support for computation offloading includes a hardware framework for  implementing and running extended memory services.
%Each application's compute offload is encapsulated in a {\em module} on the FPGA,
%with its own protection domain and virtual address space.
% (that is orthogonal to user application processes).
%These modules can directly use \sys's virtual memory data/metadata APIs and distributed operations, %, distributed operations, and 
%or implement their own counterparts but leverage \sys's general framework. %(\eg, by building 
%Thus, developing extended memory services on \sys\ is easier than on raw hardware but still flexible.

The rest of the paper will dive deep into \sys\ design and our FPGA prototype implementation.
We built five applications on top of \sys:
an image compression utility, a binary-tree index, a key-value store, a multi-version object store, and a simple data analytics service.
%We prototyped \sys's memory device with FPGA (\sysboard).
%\sys\ achieves high throughput (100\Gbps\ with FPGA prototype), low (tail) latency (XXX\mus\ end-to-end MTU round trip latency), 
%low cost (XXX\x\ energy saving), %and great extendibility,
%and \sys\ scales well with XXX. %eliminates {\em all} scalability bottlenecks in both its memory and network systems.
We compared \sys\ with vanilla RDMA, two RDMA-based disaggregated/remote memory systems~\cite{Tsai20-ATC,HERD}, 
%an FPGA-based RDMA implementation~\cite{StRoM}, 
and a software-based SmartNIC~\cite{BlueField}.
\sys\ scales much better and has orders of magnitude lower tail latency than RDMA, 
while achieving similar throughput and min latency as RDMA (even with the slower FPGA frequency in our prototype).
\sys\ also consumes 24\% to 72\% less energy than CPU-based disaggregated memory systems 
and is 2.7\x\ faster than low-power SmartNIC solutions. 






\if 0
Overall, this paper makes the following contributions.

\begin{itemize}

\item The first publicly described disaggregated memory system built with real (non-server) hardware.

\item A design that separates memory systems' data and metadata planes into hardware and software.

\item A distributed virtual memory system that integrates hardware and software in novel ways.

%\item Hardware-based distributed operation support such as migration and replication.

\item A framework to build extended memory services %on virtual memory interface
and two hardware-based distributed memory services.
% and a set of extended virtual memory APIs. 
%\item Demonstration of how real systems could use and benefit from disaggregated memory services.

%\item Two hardware-based high-level distributed memory services.
%\item Demonstration of two deployment models of disaggregated memory hardware.

\end{itemize}
\fi


==> v2-motivation.tex <==

\input{tbl-system-cmp}

\section{Memory Disaggregation}
\label{sec:motivation}

Resource disaggregation is a notion to separate different types of resources into different pools,
each of which can be independently managed and scaled.
Applications can allocate resources from any available node in a resource pool, resulting in tight resource packing. %regardless of where other types of resources sit.
Because of these benefits, % its manageability, independent scaling, and efficient resource utilization benefits,
many datacenters have adopted the idea of disaggregation, often at the storage 
layer~\cite{FACEBOOK-BRYCECANYON,FB1,SnowFlake-NSDI20,AMAZON-S3,AMAZON-EBS,Ali-SinglesDay}.
%layer~\cite{FACEBOOK-BRYCECANYON,FB1,SnowFlake-NSDI20,Decibel-NSDI17,AMAZON-S3,AMAZON-EBS,Klimovic18-ATC,RackScaleDisaggregation}.
%As a recent success story, Alibaba listed their storage disaggregation as one of the five reasons
%that enable them to serve the peak load of 544,000 orders per second on the 2019 Single's Day~\cite{Ali-SinglesDay}.
With the success of disaggregated storage and the fast developments in datacenter network speed,
researchers in both academia and industry started to seek ways to disaggregate memory 
(and persistent memory)~\cite{Lim09-disaggregate,FireBox-FASTKeynote,IntelRackScale,Lim12-HPCA,Shan18-OSDI,RAMCloud,Tsai20-ATC,AIFM,FastSwap,InfiniSwap,Semeru,Nitu18-EUROSYS}.
Different from distributed memory such as distributed shared memory~\cite{Shasta,Bennett90-PPOPP,Fleisch89-SOSP,Keleher92-ISCA,Grappa},
the disaggregated memory model has a clear notion of function separation where the memory pool hosts memory
and the compute pool executes applications.
This section, Table~\ref{tbl-system-cmp}, and Figure~\ref{fig-arch} summarize three main architecture of disaggregated memory.

\input{fig-architecture}

\subsection{Physical Disaggregated Memory}
\label{sec:pdm}

One way to build disaggregated memory is to treat it as raw, physical memory.
%\ie, client servers send read/write request with physical memory address, and the memory node directly read/write to that address without any address mapping.
We call this model {\em \pdm}.
The \pdm\ model has been adopted by a set of coherent interconnect proposals~\cite{Genz-citation,CXL-citation},
HPE's ``The Machine'' (Memory-Driven Computing) project~\cite{HP-TheMachine,THEMACHINE-HOTOS,HP-MODC-POSTER,THEMACHINE-WEB},
and two RDMA-based software systems~\cite{Tsai17-SOSP,Tsai20-ATC} 
(these systems use the OS kernel to register physical memory directly, which is a special RDMA configuration).
In order to prevent applications from accessing raw physical memory,
these solutions add an indirection layer in either hardware~\cite{Genz-citation,CXL-citation} or software~\cite{Tsai17-SOSP,Tsai20-ATC}
at \CN{}s to map client process virtual addresses (VAs)~\cite{Genz-citation,CXL-citation} or client objects~\cite{Tsai17-SOSP}/keys~\cite{Tsai20-ATC}
to physical addresses (PAs) at \MN{}s. 

There are several common problems with all the \pdm\ solutions.
First, because \MN{}s in \pdm\ are passive, raw memory, \CN{}s need multiple network round trips to access an \MN\ 
for complex operations like pointer chasing and concurrent operations that need synchronization~\cite{Tsai20-ATC}.
Second, \pdm\ requires the client side to manage disaggregated memory, which is much harder and performs worse than if management is done at the memory side.
For example, \CN{}s need to coordinate with each other or use a global controller~\cite{Tsai20-ATC} to perform tasks like memory allocation.
%and when some memory needs to be migrated from one \MN\ to another (\eg, for load balancing), 
%all the \CN{}s that have mapped this memory need to update their mappings.
%Such complex client-side memory management defeats the purpose and benefits of disaggregation (\textbf{R5}).
Third, exposing physical memory creates potential security issues. % (\textbf{R6}).
\MN{}s have to trust that \CN{}s will never access beyond their allocated physical memory regions. 
%coordination across client servers (\eg, through a global controller~\cite{Tsai20-ATC} or a distributed consensus system).
Fourth, it is difficult to build compute offloads on raw physical memory and unsafe to run them without memory protection.
Finally, all existing \pdm\ solutions require physical memory pinning at \MN{}s, causing memory wastes.
%it is also unclear how page faults will be handled.

In addition to the above common problems, none of the coherent interconnects have been actually built.
When they do, they will require new hardware at all endpoints and new switches. 
Moreover, these fabrics automatically make caches at different endpoints coherent, which is costly (because of network communication) and not always necessary.

%Recently, new cache-coherent interconnects like Gen-Z~\cite{Genz-citation} and CXL~\cite{CXL-citation}
%have been proposed to connect heterogeneous components in a rack~\cite{Genz-citation,CXL-v2} or in a server~\cite{CXL-citation,CCIX,OpenCAPI}.
%for single-machine or rack scale memory accesses.
%They usually expose a global memory space (that covers memory and accelerator memory) to applications running at the compute (client) 
%side and guarantee cache coherence among different compute and memory components.



\subsection{RDMA-Based and Messaging-Based Disaggregated Memory}
\label{sec:rdma}

The second approach, taken by many server-based disaggregated memory systems~\cite{XXX},
uses the abstraction provided by a network layer (RDMA~\cite{InfiniSwap,FastSwap,Semeru} or TCP~\cite{AIFM}).
%As discussed in \S\ref{sec:intro}, 
RDMA and TCP's symmetric architecture and connection-based, reliable transports are ill fit for memory disaggregation.
Each of them also have their own problems.
TCP or other messaging-based disaggregated memory systems first copy application objects to messages at \CN{}s
and then from messages to memory locations at \MN{}s.
These systems not only incur the performance overhead of memory copies 
but also require intensive CPU cycles to run the network transport layer,
making them unfit for memory disaggregation.
%These memory copies not only add performance overhead but also 

%RDMA is a high-speed, zero-copy, low CPU-utilization network technology 
%that has been adopted by several major datacenters~\cite{Microsoft,Alibaba}.
RDMA is not a scalable or low-cost way to build disaggregated memory systems
because of its reliance on the host CPU, MMU, and OS to run a virtual memory system.
%a host server box (CPU, MMU, and OS).
%RDMA's main issue when used for memory disaggregation is its reliance on host CPU, MMU, and OS
%and its limited scalability.
%RDMA relies on a host server's virtual memory system to manage the memory in this server.
%(\eg, for virtual and physical memory allocation, address translation, and page fault handling).
%Thus, \MN{}s can only be operated with a host server box.
A process ($P_M$) running at an \MN\ needs to allocate memory in its virtual memory address space 
and {\em register} the allocated memory (called memory region, or MR) with RDMA NIC (RNIC).
The host OS and MMU set up and manage the page table that maps $P_M{\text -}VA$ to $PA$.
%Client applications use $P_M$'s virtual memory address ($P_M{\text -}VA$) and MR information to perform RDMA read/write.
%On the \CN-side, there needs to be an extra level of indirection to first translate application abstraction to the $P_M{\text -}VA$ and MR combination.
%On the \MN-side, RNICs rely on host OS and MMU to manage page tables that map $P_M{\text -}VA$ to $PA$ (physical memory address).
To avoid always accessing host memory for address mapping, RNICs cache PTEs,
but when more PTEs are accessed than what this cache can hold, RDMA performance degrades significantly (Figure~\ref{fig-pte-mr} and \cite{FaRM,Tsai17-SOSP}).
Similarly, RNICs cache MR metadata and incur degraded performance when the cache is filled.
%Thus, RDMA has serious performance issues with either large memory (PTEs) or many disjoint memory regions (MRs).
Moreover, RDMA uses a slow way to support on-demand allocation: RNICs interrupt the host OS on the first accesses for handling the page faults.
From our experiments, a faulting RDMA access is 14100\x\ slower than a no-fault access.
%to handle page faults, which is extremely slow (14100\x\ slower than a no-fault access from our experiments).

To mitigate these performance and scalability issues of RDMA, most RDMA-based systems today~\cite{FaRM,XXX} 
preallocate a big MR with huge page and pin it in physical memory, 
which results in inefficient memory space utilization.
Even with this approach, there can still be a scalability issue,
as RDMA uses MR as the protection domain and need to create one MR for each client that needs isolation.
Moreover, each client usually needs another level of indirection to map from its interface (\eg, VA of the client process)
to $P_M{\text -}VA$ and MR.
%RNICs rely on host OS and MMU to manage page tables.
As \sys\ demonstrates, we can solve all these performance, scalability, and space utilization issues of RDMA 
when managing the virtual memory system at \MN\ hardware, %removing the reliance on host-server virtual memory system,
%we can achieve scalable, low-tail-latency performance and efficient memory utilization at the same time. 

%Similarly, RNICs cache MR metadata and connection (QP) metadata,
%and they too cause scalability issues.
%and \CN{}s need to communicate with a proxy process at an \MN{}, which does the memory allocation and registration tasks.
%A client application's abstraction needs to first map to this proxy process' virtual memory address at a \CN{},
%which is then mapped to physical memory address at \MN{}s.
%With RDMA, a process running at an \MN\ server first needs to {\em register} a memory 
%region (MR) with RDMA NIC (RNIC) using its own virtual memory address.
%disaggregated memory exposes the virtual memory address spaces of processes running at an \MN\ server (\mnva);
%This address then needs to be passed to client processes running at \CN{}s to be used to perform RDMA read/write.
%Application processes' virtual memory addresses or objects are first mapped to \mnva{}s at \CN,
%and \mnva{}s are then mapped to physical memory addresses at \MN{}s.
%This two-level indirection is not only redundant but also results in the reliance on host CPU, MMU, and OS for providing virtual memory system features.
%Moreover, RDMA supports on-demand memory allocation by interrupting the host CPU to let the OS handle page faults,
%which is extremely slow (XXX\x\ slower than a no-fault access).
%As another example, it is slow for RNICs to access page tables and MR metadata stored in DRAM over PCIe.
%To speed up address translation, RNICs cache PTEs and MR metadata,
%but when the cache is filled up, RDMA performance drops significantly.

Apart from RDMA's various memory-management-related issues, 
RDMA suffers a few network-related problems: a QP (connection) scalability issue (Figure~\ref{fig-conn})
and a ``head-of-line blocking'' issue because of its reliance on PFC (Priority Flow Control)~\cite{DCQCN,AliNSDI21}.
1RMA~\cite{1RMA} is a recent network solution that uses a connection-less, solicitation-based protocol to solve these issues.
However, 1RMA's memory management model is essentially the same as RDMA and incurs the same issue of relying on the host OS to perform virtual memory tasks~\cite{1RMA-comm-w-author}.
\sys\ solves not only the same RDMA networking issues as 1RMA but also RDMA's memory-related issues,
and unlike 1RMA, \sys\ is a full disaggregated memory system with computation offloading support.
% but avoids the extra RTT in 1RMA's ``remote-request-to-read'' write mechanism~\cite{1RMA}.
%In addition, \sys\ avoids RDMA's other issues such as QP (connection) scalability and PFC head-of-line blocking.
%have to either allocate and ping physical memory before using it (and thus waste memory)
%Moreover, 
%More important, 1RMA is not a disaggregated memory system that offers virtual memory support,
%and it requires new NIC hardware at all participating nodes.


%\subsection{Virtual Disaggregated Memory}
\subsection{Our Proposal: Hardware-Based Smart Virtual Disaggregated Memory}
\label{sec:vdm}

Existing disaggregated memory solutions either manage memory at the client side (\pdm), 
which causes high communication overhead and security concerns, 
or rely on a host server to run a virtual memory system (RDMA- and messaging-based),
which has tail latency, scalability, and cost issues.
We believe that disaggregated memory should be managed at the memory side behind a per-client virtual memory abstraction, 
but without the reliance on a host server and with the support for computation offloading.
%With a per-client virtual memory abstraction, 
%application-level programs and low-level systems like databases and JVM can all sit on \sys\ with each of them properly isolated,
%and the physical location of disaggregated memory can be transparent and thus non-contiguous and moved around.
By building a hardware-based ``smart'' virtual disaggregated memory system,
we can achieve low-latency performance, scalability, efficient memory utilization, low cost, and ease of management,
as what the rest of this paper will show.

%The abstraction we believe to be the best fit for memory disaggregation is a virtual memory interface that is facing client processes running at \CN{}s.
%With this abstraction, disaggregated memory can be managed at \MN{}s, which is more efficient and flexible than at \CN{}s (\S\ref{sec:intro} and \S\ref{sec:pdm}).
LegoOS~\cite{Shan18-OSDI}, an operating system designed for resource disaggregation, 
also advocates for managing memory at where memory is (called mComponent in LegoOS).
% is the only disaggregated memory system that adopts this abstraction and manages memory at \MN{}s.
However, LegoOS uses software to build the virtual memory system at mComponents, 
which has a stark difference from a hardware-based virtual memory system. 
In fact, we started our virtual memory design from LegoOS's but ended up finding 
that none of its design or implementation fit a hardware environment. 
%have to redesign every factor of it.
%still relies on host CPU and cannot be easily adapted to a hardware-based virtual memory system.
Moreover, LegoOS has no computation offloading support, 
and it uses RDMA for its network communication and inherits RDMA's limitations.

It is worth noticing that %\sys\ is a versatile system that can either 
memory disaggregation solutions that operate at higher levels,
\eg, language runtime~\cite{Semeru}, data-structure library~\cite{AIFM}, swap system~\cite{InfiniSwap,FastSwap}, %\fixme{anything else?},
can sit above the \sys\ layer and are orthogonal to our work. 
They can be ported to \sys\ by replacing the RDMA-/messaging-based abstraction to \sys's virtual memory abstraction. % (Figure~\ref{fig-usage} U3).

%\subsection{Active Disaggregated Memory}
%\label{sec:offload}



\if 0
\subsection{Requirements of Memory Disaggregation}
Many applications can benefit from disaggregated memory, and their usages can be categorized into two types:
as dynamically allocated memory space (\eg, as part of a heap~\cite{Semeru}, as a swap space~\cite{InfiniSwap}) during the execution of an application,
and as the cache of a data store~\cite{XXX} or the data store itself~\cite{RAMCloud}.
In general, memory disaggregation has the following requirements.

\stepcounter{reqs}
\boldpara{R\arabic{reqs}: Low cost and easy deployment.}
Although disaggregated memory pool can be built with regular servers 
(in fact, most of today's disaggregated memory solutions~\cite{AIFM,FarMem,InfiniSwap,Semeru} are server-based),
it is much cheaper to build and run standalone disaggregated memory devices without a server box or a CPU.
To ease the adoption of disaggregated memory in current datacenters, ideally, there should be no hardware change or addition at client servers.

\stepcounter{reqs}
\boldpara{R\arabic{reqs}: Low-latency and high-throughput.}
Accesses to disaggregated memory are over the network, which is inevitably slower than accessing local memory.
Despite this nature, memory disaggregation should still offer attractive performance, and by offering more (but slower) memory,
overall application performance could be better than with just local memory.
Specifically, when used as dynamically allocated memory, disaggregated memory should deliver low latency so as not to slow down application execution much.
When it is used as (cache of) data store, throughput is more important, 
and accesses to disaggregated memory should reach network line rate.

\stepcounter{reqs}
\boldpara{R\arabic{reqs}: Low tail latency and predictable performance.}
One of the obstacles to adopting disaggregated memory is the fear for unpreditable performance and much worse tail latency than local memory. %, \eg, during network congestion
In addition to network unstability, we found that memory systems could also contribute to long tails with today's RDMA-based systems (\S\ref{sec:}).
Having predictable, bounded performance and low tail latency would be one key to the successful adoption of memory disaggregation in data centers,
where SLAs are important.

\stepcounter{reqs}
\boldpara{R\arabic{reqs}: Scale with clients and memory.}
To fully exploit the resource-utilization benefit of disaggregation, we should allow many client servers and client processes running on them to access and share a memory device.
At the same time, each memory device could host hundreds GBs to few TBs of memory that is expected to be close to fully utilized (and thus bringing down the number of 
memory devices and total cost of a cluster).
Furthermore, we should have no restriction on how applications use the memory, which could result in many disjoint memory regions.
Thus, disaggregated memory should scale with client servers, client processes, memory size, and memory regions.
%each client process should be able to access large amounts of memory and many disjoint memory regions 
%scale with client servers, client processes, memory size, memory regions

\stepcounter{reqs}
\boldpara{R\arabic{reqs}: Independent resource pool management.}
A major reason behind the successful adoption of disaggregated storage at production scale and the traction of disaggregation in general
is its ease of management, as it is more flexible to manage disaggregated resource pools independently at where the resource is.
Memory disaggregation should also follow the practice by managing the disaggregated memory pool.
Datacenter operators can then configure disaggregated memory pool (\eg, adding replication, migrating data across memory nodes)
without affecting other pools.

\stepcounter{reqs}
\boldpara{R\arabic{reqs}: Secure access.}
When deployed in datacenters, it is important to protect disaggregated memory from undesired or malicious accesses.
Disaggregate memory can be shared by many client servers and applications over the network.
It should provide at least the same level of safety guarantees as today's normal (local) memory
and potentially also guard against new security threasts such as side channel attacks over the network~\cite{Tsai19-Security}.
%when shared across side channel attacks~\cite{Meltdown,Spectre}

\stepcounter{reqs}
\boldpara{R\arabic{reqs}: Efficient, easy, and flexible computation offloading.}
%\boldpara{R\arabic{reqs}: Extendible.}
%With the fast development of datacenter applications, hardware, and network, a good memory disaggregation solution should be flexible and extendible,
for example, to support more advanced APIs like pointer chasing~\cite{StRoM,AIFM},
to offload some application logic to memory devices~\cite{AIFM,XXX},
or to plug different network transports~\cite{Homa,NDP,pFabric,XXX} and congestion control algorithms~\cite{Swift,XXX}.

%\stepcounter{reqs}
%\boldpara{R\arabic{reqs}: Easy and cheap to deploy.}
%opportunity
%asymmetric
%application aware of disaggregated memory
\fi


\if 0
%The reason behind the \pdm\ model's issues is its physical abstraction of disaggregated memory.
%Thus, we believe that disaggregate memory should expose a \textit{virtualized} memory abstraction,
%and memory management and address mapping should happen at the memory pool, not the compute pool (client servers).
%By hiding the physical nature of disaggregated memory under a virtual abstraction,
%disaggregated memory can have the same benefits as what traditional virtual memory system provide, 
%such as on-demand allocation (paging) and protected accesses across different applications.
%By performing memory management at the memory node, we can avoid orchestration across client servers
%and transparently perform tasks like replication and migration.
%Both \sys\ and RDMA offer a virtualized disaggregated (remote) memory abstraction.
%However, the virtualized view of them are completely different, and as we will show next, RDMA has many issues when used for memory disaggregation.
%As we will show shortly, RDMA cannot meet these requirements and is an ill fit for memory disaggregation.


%This section discusses related topics 
%and motivates our work. %existing proposals and attempts to build remote memory
%and motivates programmable hardware-based disaggregated memory.
%We also cover related works in this section.

\subsection{Non-Disaggregated Remote Memory}
\label{sec:remotemem}

The idea of using non-local machine's memory dates back to the early 90s when research in 
distributed shared memory (DSM)~\cite{Shasta,Bennett90-PPOPP,Fleisch89-SOSP,Keleher92-ISCA} 
and distributed operating systems~\cite{Sprite88,Amoeba90} boomed.
Recent years have seen a rise of new interests in this idea because of datacenter network improvements~\cite{Aguilera17-SOCC}.
Several RDMA-based distributed memory systems have been proposed %in recent years
including Grappa~\cite{Nelson15-ATC}, FaRM~\cite{FaRM}, and Hotpot~\cite{Shan17-SOCC}.
%There are mainly two forms of using non-local (remote) machine's memory.
These systems use a machine's memory for both applications running locally and on remote machines.
Each machine manages its own memory and runs application processes.
Similar to traditional DSM systems, these systems require complex and costly consistency protocols for concurrent accesses.
Moreover, % important, %memory in these systems is not disaggregated 
they lack the benefits of disaggregation. % (see below).
%The second type reserves some memory space exclusively for remote accesses.
%To use these systems in a cluster setting, another distributed software system is usually needed on top of them.

\subsection{Resource Disaggregation}
\label{sec:disaggregation}

Resource disaggregation is a notion to separate different types of resources into different pools,
each of which can be independently managed and scaled.
Applications can allocate resources from any available node in a resource pool, resulting in tight resource packing. %regardless of where other types of resources sit.
Because of these benefits, % its manageability, independent scaling, and efficient resource utilization benefits,
many datacenters have adopted the idea of disaggregation, often at the storage 
layer~\cite{FACEBOOK-BRYCECANYON,FB1,SnowFlake-NSDI20,AMAZON-S3,AMAZON-EBS,Ali-SinglesDay}.
%layer~\cite{FACEBOOK-BRYCECANYON,FB1,SnowFlake-NSDI20,Decibel-NSDI17,AMAZON-S3,AMAZON-EBS,Klimovic18-ATC,RackScaleDisaggregation}.
%As a recent success story, Alibaba listed their storage disaggregation as one of the five reasons
%that enable them to serve the peak load of 544,000 orders per second on the 2019 Single's Day~\cite{Ali-SinglesDay}.

With the success of disaggregated storage and the fast developments in datacenter network speed,
researchers in both academia and industry started to seek ways to disaggregate memory 
(and persistent memory)~\cite{Lim09-disaggregate,FireBox-FASTKeynote,IntelRackScale,Lim12-HPCA,Shan18-OSDI,RAMCloud,Tsai20-ATC}.
Disaggregated memory proposals so far have taken two main approaches.
The first type treats the disaggregated memory layer as a {\em passive} party (raw, physical memory space with no processing power);
the compute pool manages the memory pool and provides high-level services to applications~\cite{HP-TheMachine,Tsai20-ATC,Lim09-disaggregate,Nitu18-EUROSYS}.
%that requires the compute pool for further management and high-level interface, 
The main problem of passive disaggregation is the excessive network RTTs needed when completely separating processing and memory.
% in passive disaggregated memory results in excessive RTTs and performance loss.

The second type (active disaggregated memory) organizes the disaggregated memory pool with regular servers and runs all or part of management software 
at these servers' CPUs~\cite{InfiniSwap,NAMDB,Kalia14-RDMAKV,Aguilera18-ATC}. 
%Recent proposals in this type include RDMA-based remote memory swap system~\cite{InfiniSwap}, remote database system~\cite{NAMDB}, 
%remote key-value store~\cite{Kalia14-RDMAKV}, and remote memory system with file interfaces~\cite{Aguilera18-ATC}.
%hey all run their memory systems on regular machines and use those machines' CPU to manage the memory spaces.
Co-locating management with memory reduces network RTTs.
However, these server-based solutions increase owning and energy cost, with full servers and large amounts of CPU cycles at the memory layer.
Moreover, the number of CPU cores limits the amount of parallel memory requests a memory server can handle.
An alternative way of building active disaggregated memory is to run management software in low-power cores.
However, recent work shows that low-power cores cannot meet the high-bandwidth and low-latency demands of memory systems~\cite{Tsai20-ATC}.

\phdm\ solves the problems of both these two existing disaggregated memory models.
By managing memory and providing distributed memory services in hardware at \MN{}s,
\phdm\ can achieve great performance, low network bandwidth consumption, and low monetary and energy cost.

LegoOS~\cite{Shan18-OSDI} is a distributed OS that takes a {\em partially} active disaggregation approach. 
%designed for resource disaggregation. %, which also advocates for managing resources at the resource nodes.
It runs a virtual memory system at its disaggregated memory pool and exposes a virtual memory interface to the compute pool.
%However, a virtual memory system is all what LegoOS' memory layer runs.
To support higher-level memory services, LegoOS still needs to add a software layer at the compute side.
More important, LegoOS has no real hardware design or implementation.
%runs all management in software on regular servers that are emulated as resource devices.
HPE's ``The Machine'' (Memory-Driven Computing) project~\cite{HP-TheMachine,THEMACHINE-HOTOS,HP-MODC-POSTER,THEMACHINE-WEB}
is another proposal that adopts the partially active disaggregation approach.
It separates a pool of DRAM/NVM from a pool of SoCs with a special interconnect inside a rack. % through a special interconnect~\cite{Genz-citation}. 
Memory instructions running at SoCs are transparently translated to access the DRAM/NVM pool,
and the translation is performed either at the interconnect~\cite{Genz-citation} or at the memory pool.
Similar to LegoOS, the Machine still needs extra software running at the SoC pool to provide high-level memory services.
Moreover, neither its design nor its maturity is known to the public.
%The DRAM/NVM pool provides a global memory address space,
%which requires extra software running at the SoC pool to manage and . % in, and use the memory pool.

\subsection{RDMA and Other Network Technologies}
\label{sec:rdma}

Datacenter network speed has increased dramatically in the past decade.
%Most datacenters now run on 10\Gbps/server or 40\Gbps/server networks~\cite{CatapultV1,Facebook-10GDatacenter},
%with 100\Gbps\ and 200\Gbps\ networks on the horizon~\cite{Facebook-100G,Mellanox200Gbps}.
%Meanwhile, network RTT can be as low as 1\mus\ for a single hop~\cite{Mellanox-Switch}.
High-bandwidth, low-latency networks give rise to a surge of interest in exploring remote or disaggregated 
resources~\cite{FaRM,FireBox-FASTKeynote,Shan18-OSDI,HP-TheMachine}.
%Network's much faster frequency speedup than CPU's~\cite{XXX} also motivated offloading various application and 
%I/O functionalities to hardware.
%Both these hardware trends are in line with what we propose in \phdm.

A high-speed network technology that several major datacenters have adopted~\cite{AZURE-RDMA,ALIBABA-RDMA} is
{\em Remote Direct Memory Access} (RDMA),
%RDMA supports both {\em one-sided} and {\em two-sided} communication to remote memory.
%One-sided RDMA allows one machine to directly read and write another machine's memory without involving the latter's CPU.
%Two-sided RDMA works like traditional messaging, involving both sender and receiver CPU.
which is the communication media adopted by most remote memory systems. % use RDMA as the communication media.
%with one-sided RDMA being used by systems where remote memory are managed by local (compute) machines~\cite{DPM}
%and two-sided RDMA used by systems where each machine manages its own memory~\cite{Kalia14-RDMAKV,Mitchell13-ATC}.
%With the help of one-sided RDMA and other one-sided network technologies~\cite{GenZ},
%several software systems have been proposed to treat 
%Albeit its superior performance, RDMA's limited interface is too restrictive for most applications,
Although several recent proposals of hardware~\cite{StRoM,Aguilera-FarMemory} and software~\cite{Tsai17-SOSP,HyperLoop} extensions to RDMA made it more flexible and performant, 
RDMA is still an ill fit for memory disaggregation.
The RDMA protocol and its implementation are both tightly bound with the processor that co-locates with the memory.
At least a process running on this processor needs to perform virtual memory allocation 
and registration through an OS and then share the allocated virtual memory addresses
with other (client) servers that wish to access the allocated memory. 
Essentially, RDMA's abstraction is a {\em host-server-centric} memory view.
What fits disaggregated memory and what \phdm\ provides is a {\em client-centric} memory view 
where client applications running on a server can directly access remote memory without the need to contact or maintain 
any additional processes or OSs running at the memory side.
Moreover, \phdm\ is a system-level design that has built-in distributed support, while RDMA is just a network layer that needs another software distributed system. 
%a client-side address space in \phdm\ could span multiple \MN{}s. %memory nodes.
%This client virtual address space can also span multiple \MN{}s.

Recently, new cache-coherent interconnects like Gen-Z~\cite{Genz-citation} and CXL~\cite{CXL-citation}
have been proposed for single-machine or rack scale memory accesses.
They expose a global memory space to applications running at the compute (client) 
side and guarantee cache coherence among applications and memory.
They are low-level, physical-layer solutions for accessing disaggregated memory.
With additional software systems, they could be used to build passive disaggregated memory.
\phdm's active disaggregated memory model saves network RTTs and client-side CPU cycles.
Moreover, the need to mainain cache coherence limits the scalability of these interconnects, and they require the replacement of existing datacenter network infrasturcture.
\phdm\ does not have cache-coherence scalability bottlenecks
and builds on Ethernet and can directly be deployed in today's datacenters.
%Rack-scale cache-coherent interconnects like CXL and Gen-Z provide a hardware layer to access disaggregated memory. 
%Software layer needs to be added on top (at the CPU side) to manage the disaggregated memory space.

\subsection{HADM Benefits and Use Cases}

The \phdm\ model offers several benefits over existing proposals. 
%that are key to meeting today's datacenter needs.
Unlike non-disaggregated remote memory, 
\phdm's separate, self-contained disaggregated memory layer is easy to configure, manage, and scale.
Compared to software-based approaches, 
\phdm\ can achieve 
%with hardware-based implementation, remote memory services can achieve
high-bandwidth, low-latency performance 
and sustain large concurrent loads
without paying the high costs of full servers.
Unlike passive disaggregated memory,
%By offering high-level distributed memory services, 
applications can build different remote memory services and/or offload
their near-data computation to the memory pool, 
improving performance and reducing CPU cycles.
%easily use remote memory without 
%worrying about its distributed nature or dealing with low-level interfaces.
%Finally, programmable hardware enables the reuse of the same hardware for different 
%types of memory services, yielding faster and cheaper deployment. %option than ASIC.

Many types of applications can make use of \phdm.
For example, applications or libraries can store large in-memory data structures 
like hash tables and tree indices at \phdm's memory pool and offload operations
like hash lookup and tree traversal to move computation closer to data.
More advanced types of application offloading are also possible, such as data 
processing and data analytics.
Applications can also use the memory layer of \phdm\ as a location to cache storage 
data or to share data across different compute nodes, 
\eg, storage-data caching or shared states for serverless computing systems.
Finally, OS and low-level systems software can build more functionalities like remote swap over \phdm\
and offer applications transparent accesses to remote memory.
See Appendix for further discussion.


\fi


\if 0
\sys\ is also different from previous computation offloading systems in terms of its hardware choice.
Previous solutions use either FPGA or ARM-based SoC to build their smart devices.
%with most of them also include a full NIC on board.
\MN{}s in \sys\ include both FPGA and ARM 
and use them for different planes. %, with the former used for the data plane and the latter used for the control plane.
%\sys\ integrates all the data path, including a lean network stack, on a single FPGA chip,
%while moving all the control plane and metadata operations to the SoC.
In doing so, \sys\ could achieve the best performance, cost, and programmability
combination that fits the need of a remote memory system.
%FPGA has seen an increasing adoption in industry~\cite{XXX} and more research interests~\cite{XXX} in recent years.
%Among the many FPGA-based systems, KV-Direct~\cite{KVDIRECT} and Catapult~\cite{XXX} are most relevant to \sys.
\fi

\if 0
Among all existing computation offloading solutions, three are the most relevant to \sys. 
KV-Direct~\cite{KVDIRECT} is a remote key-value store built on FPGA.
%Similar to \sys, it also integrates a lightweight network stack on the FPGA chip.
Unlike \sys, it targets a non-disaggregated environment and 
relies on the host CPU to perform metadata tasks such as memory allocation.
StRoM~\cite{StRoM} is a recent hardware proposal that includes a full RoCE (RDMA-over-Converged-Ethernet) network stack
and several high-level APIs like pointer chasing on an FPGA.
Although StRoM extends RDMA's restricted APIs to a more feature-rich interface,
it still has the same host-based memory view like RDMA (\S\ref{sec:rdma}).
Moreover, it has no distributed systems support.
Catapult~\cite{Catapult,CatapultV1} is a general-purpose distributed FPGA computation-offloading platform developed and deployed at Microsoft.
%which has been used for network-function offloading~\cite{AccelNet}, deep-learning inference~\cite{Brainwave}, and Bing search~\cite{CatapultV1}.
%Although Catapult is also a distributed FPGA-based platform, 
Different from \sys, Catapult is designed for a non-disaggregated environment 
and targets general computation offloading instead of memory management/services.
\fi


\if 0
Conceptually, the \phdm\ model could be built using any programmable hardware technologies.
For example, a SmartNIC could be extended to a programmable disaggregated memory device by attaching some memory chips to it.
Processor-based SmartNICs usually attach an ARM-based SoC or a small CPU to a NIC~\cite{BLUEFIELD,BROADCOM-SMARTNIC}.
Software can be easily deployed in the processor.
However, our experiments show that the processor cannot meet the performance requirements of high-speed network.
Hardware-based SmartNICs attach an FPGA chip to a NIC~\cite{INNOVA,SOLARFLARE-FPGA}.
\sys's hardware architecture is close to these SmartNICs, both using FPGA as programmable hardware (and thus could easily be modified to run on them).
Differently, \sys\ does not use a separate NIC and integrates the network stack with the memory services, 
saving both monetary cost and the performance overhead of communicating between two chips.
\fi


